Towards Precision Therapy in Hepatocellular Carcinoma: A Clinical-Reasoning LLM for Risk Stratification and Treatment Guidance

Hepatocellular carcinoma (HCC) is a common malignancy and a leading cause of cancer-related mortality. Current guidelines and staging systems provide coarse categories, but often miss within-stage heterogeneity and the clinical context in electronic medical records (EMRs). We present HCC-STAR (Hepatocellular Carcinoma Staging, Treatment And pRognosis), a clinically aligned large language model that reads routine EMR narratives and jointly outputs risk score-based staging, ranked guideline-consistent treatments with evidence-based rationales, and individualized survival estimates. We curated about 30,000 HCC cases from SEER and expanded them into EMR-style narrative training data using a clinician-validated, prompt-based augmentation workflow. On this corpus, we developed a knowledge-aligned reasoning framework optimized with a step-verifiable composite reward, moving beyond text-level memorization of clinical guidelines. In a multi-center cohort of 6,668 patients from 12 hospitals in China, HCC-STAR achieved state-of-the-art performance in treatment recommendation and risk stratification compared with clinical guidelines and competitive models, including GPT-5 and Gemini-2.5 Pro. Hypothetical overall-survival analysis showed a median survival of 51 months under adherence to HCC-STAR recommendations, compared with 29 and 32 months under BCLC and CNLC. In clinician-centric evaluations, blinded hepatobiliary specialists rated HCC-STAR's reasoning and evidence-based justifications as trustworthy. The model surpassed resident and attending physicians in treatment accuracy and helped physicians make more accurate decisions faster when used as an assistant. These findings support HCC-STAR as a reliable and verifiable decision-support system for risk stratification and precision therapy in HCC.

==> baseline_final_external.tex <==
    % Preamble needed:
    % \usepackage{pdflscape,longtable,booktabs,array}
    % \usepackage{caption} % optional for caption*
    % Example usage: place this entire environment where you want the table.
    \begin{landscape}
    \begin{center}
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.25}
    \begin{longtable}{p{5.2cm}p{3.0cm}}}}}}}}}}}}}
    \caption{Baseline characteristics of patients in the external multi-center HCC cohort (final test set after exclusions)}\label{tab:baseline_final_external}\\
\toprule
Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
\midrule
\endfirsthead
\caption*{Baseline characteristics of patients in the external multi-center HCC cohort (final test set after exclusions) (continued)}\\
\toprule
Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
\midrule
\endhead
\midrule
\multicolumn{13}{r}{\small Continued on next page}\\
\bottomrule
\endfoot
\bottomrule
\endlastfoot

     & N=412 & N=1941 & N=61 & N=817 & N=143 & N=314 & N=249 & N=47 & N=76 & N=18 & N=56 & N=56 \\
Sex, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
female & 55 (13.3\%) & 397 (20.5\%) & 11 (18.0\%) & 104 (12.7\%) & 33 (23.1\%) & 55 (17.5\%) & 40 (16.1\%) & 11 (23.4\%) & 10 (13.2\%) & 2 (11.1\%) & 9 (16.1\%) & 8 (14.3\%) \\
male & 357 (86.7\%) & 1544 (79.5\%) & 50 (82.0\%) & 713 (87.3\%) & 110 (76.9\%) & 259 (82.5\%) & 209 (83.9\%) & 36 (76.6\%) & 66 (86.8\%) & 16 (88.9\%) & 47 (83.9\%) & 48 (85.7\%) \\
Age (years), (median [IQR]) & 56.5 [50.0;63.0] & 60.0 [53.0;66.0] & 57.0 [49.0;62.0] & 57.0 [48.0;64.0] & 60.0 [53.0;67.0] & 61.0 [53.0;68.0] & 57.0 [48.0;66.0] & 52.0 [41.5;59.0] & 61.0 [51.0;69.0] & 52.5 [45.0;60.0] & 60.0 [51.5;65.0] & 54.5 [45.8;65.2] \\
BMI (kg/m2), (median [IQR]) & 23.8 [21.5;26.1] & 24.2 [22.3;26.8] & 22.6 [20.9;24.0] & 23.7 [21.7;26.3] & 23.5 [21.4;25.9] & 23.5 [20.3;26.8] & 23.7 [21.3;25.8] & 23.5 [20.7;25.6] & 23.9 [22.4;26.1] & 23.7 [22.1;25.6] & 24.0 [21.2;26.8] & 24.3 [20.4;26.0] \\
Diabetes, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 271 (70.0\%) & 1564 (80.6\%) & 52 (85.2\%) & 646 (82.7\%) & 104 (89.7\%) & 252 (80.3\%) & 211 (84.7\%) & 41 (87.2\%) & 57 (75.0\%) & 15 (83.3\%) & 39 (69.6\%) & 51 (91.1\%) \\
Yes & 116 (30.0\%) & 377 (19.4\%) & 9 (14.8\%) & 135 (17.3\%) & 12 (10.3\%) & 62 (19.7\%) & 38 (15.3\%) & 6 (12.8\%) & 19 (25.0\%) & 3 (16.7\%) & 17 (30.4\%) & 5 (8.93\%) \\
Hypertension, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 275 (71.1\%) & 1264 (65.1\%) & 45 (75.0\%) & 627 (80.3\%) & 96 (73.3\%) & 201 (64.0\%) & 198 (79.5\%) & 39 (83.0\%) & 53 (69.7\%) & 14 (77.8\%) & 41 (73.2\%) & 43 (76.8\%) \\
Yes & 112 (28.9\%) & 677 (34.9\%) & 15 (25.0\%) & 154 (19.7\%) & 35 (26.7\%) & 113 (36.0\%) & 51 (20.5\%) & 8 (17.0\%) & 23 (30.3\%) & 4 (22.2\%) & 15 (26.8\%) & 13 (23.2\%) \\
Cirrhosis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 47 (11.9\%) & 424 (21.9\%) & 34 (55.7\%) & 402 (55.4\%) & 14 (9.86\%) & 137 (43.6\%) & 99 (39.8\%) & 13 (27.7\%) & 9 (11.8\%) & 6 (33.3\%) & 15 (26.8\%) & 7 (12.5\%) \\
Yes & 348 (88.1\%) & 1510 (78.1\%) & 27 (44.3\%) & 323 (44.6\%) & 128 (90.1\%) & 177 (56.4\%) & 150 (60.2\%) & 34 (72.3\%) & 67 (88.2\%) & 12 (66.7\%) & 41 (73.2\%) & 49 (87.5\%) \\
Chronic liver disease, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 23 (5.65\%) & 188 (9.69\%) & 0 (0.00\%) & 118 (15.1\%) & 11 (8.21\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
HBV & 315 (77.4\%) & 1438 (74.1\%) & 35 (67.3\%) & 591 (75.7\%) & 119 (88.8\%) & 234 (74.5\%) & 213 (85.5\%) & 42 (89.4\%) & 65 (85.5\%) & 18 (100\%) & 48 (85.7\%) & 47 (83.9\%) \\
HBV+HCV & 2 (0.49\%) & 12 (0.62\%) & 0 (0.00\%) & 8 (1.02\%) & 0 (0.00\%) & 2 (0.64\%) & 1 (0.40\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
HCV & 19 (4.67\%) & 133 (6.85\%) & 0 (0.00\%) & 22 (2.82\%) & 4 (2.99\%) & 0 (0.00\%) & 7 (2.81\%) & 0 (0.00\%) & 4 (5.26\%) & 0 (0.00\%) & 6 (10.7\%) & 2 (3.57\%) \\
Others & 48 (11.8\%) & 170 (8.76\%) & 17 (32.7\%) & 42 (5.38\%) & 0 (0.00\%) & 78 (24.8\%) & 28 (11.2\%) & 5 (10.6\%) & 7 (9.21\%) & 0 (0.00\%) & 2 (3.57\%) & 7 (12.5\%) \\
ECOG PS, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
0 & 249 (60.4\%) & 1197 (61.7\%) & 35 (57.4\%) & 450 (55.1\%) & 86 (60.1\%) & 314 (100\%) & 55 (22.1\%) & 20 (42.6\%) & 38 (50.0\%) & 2 (11.1\%) & 29 (51.8\%) & 27 (48.2\%) \\
1 & 127 (30.8\%) & 744 (38.3\%) & 24 (39.3\%) & 322 (39.4\%) & 45 (31.5\%) & 0 (0.00\%) & 177 (71.1\%) & 26 (55.3\%) & 38 (50.0\%) & 13 (72.2\%) & 19 (33.9\%) & 24 (42.9\%) \\
2 & 36 (8.74\%) & 0 (0.00\%) & 2 (3.28\%) & 45 (5.51\%) & 12 (8.39\%) & 0 (0.00\%) & 17 (6.83\%) & 1 (2.13\%) & 0 (0.00\%) & 3 (16.7\%) & 8 (14.3\%) & 5 (8.93\%) \\
Child-Pugh stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
A & 246 (59.7\%) & 1705 (87.8\%) & 51 (83.6\%) & 606 (74.2\%) & 123 (86.0\%) & 299 (95.2\%) & 245 (98.4\%) & 47 (100\%) & 59 (77.6\%) & 18 (100\%) & 46 (82.1\%) & 49 (87.5\%) \\
B & 118 (28.6\%) & 236 (12.2\%) & 7 (11.5\%) & 211 (25.8\%) & 20 (14.0\%) & 12 (3.82\%) & 4 (1.61\%) & 0 (0.00\%) & 17 (22.4\%) & 0 (0.00\%) & 10 (17.9\%) & 7 (12.5\%) \\
C & 48 (11.7\%) & 0 (0.00\%) & 3 (4.92\%) & 0 (0.00\%) & 0 (0.00\%) & 3 (0.96\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
mALBI\_stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
Grade 1 & 61 (17.2\%) & 1464 (76.3\%) & 24 (39.3\%) & 274 (39.3\%) & 59 (41.3\%) & 207 (65.9\%) & 190 (76.3\%) & 31 (66.0\%) & 26 (34.2\%) & 10 (55.6\%) & 32 (57.1\%) & 26 (46.4\%) \\
Grade 2a & 62 (17.5\%) & 283 (14.8\%) & 15 (24.6\%) & 193 (27.7\%) & 31 (21.7\%) & 72 (22.9\%) & 46 (18.5\%) & 9 (19.1\%) & 15 (19.7\%) & 6 (33.3\%) & 6 (10.7\%) & 10 (17.9\%) \\
Grade 2b & 181 (51.1\%) & 163 (8.50\%) & 20 (32.8\%) & 211 (30.2\%) & 52 (36.4\%) & 33 (10.5\%) & 12 (4.82\%) & 6 (12.8\%) & 29 (38.2\%) & 2 (11.1\%) & 16 (28.6\%) & 19 (33.9\%) \\
Grade 3 & 50 (14.1\%) & 8 (0.42\%) & 2 (3.28\%) & 20 (2.87\%) & 1 (0.70\%) & 2 (0.64\%) & 1 (0.40\%) & 1 (2.13\%) & 6 (7.89\%) & 0 (0.00\%) & 2 (3.57\%) & 1 (1.79\%) \\
WBC (109/L), (median [IQR]) & 3.91 [2.83;5.21] & 5.11 [4.08;6.27] & 5.30 [4.35;6.84] & 5.48 [4.10;7.14] & 4.80 [3.70;6.10] & 5.60 [4.50;7.00] & 5.54 [4.51;6.97] & 4.94 [4.10;5.97] & 4.80 [3.88;6.15] & 5.70 [4.85;7.55] & 5.20 [3.55;6.43] & 4.55 [3.10;5.85] \\
NEUT (109/L), (median [IQR]) & 2.66 [1.73;4.72] & 2.86 [2.15;3.73] & 3.70 [2.62;6.24] & 3.40 [2.40;4.80] & 2.70 [2.00;3.75] & 3.58 [2.66;4.65] & 2.99 [2.40;4.02] & 3.08 [2.24;4.03] & 3.15 [2.40;4.60] & 3.13 [2.77;5.44] & 3.70 [2.50;4.73] & 3.25 [2.28;4.50] \\
LYMPH (109/L), (median [IQR]) & 0.64 [0.38;1.11] & 1.54 [1.19;1.95] & 1.00 [0.70;1.42] & 1.26 [0.86;1.75] & 1.26 [0.90;1.75] & 1.49 [1.07;1.86] & 1.68 [1.31;2.12] & 1.33 [1.06;1.46] & 0.90 [0.70;1.40] & 1.68 [1.40;2.05] & 1.10 [0.70;1.55] & 0.85 [0.60;1.20] \\
RBC (1012/L), (median [IQR]) & 3.75 [3.13;4.31] & 4.62 [4.23;4.98] & 4.01 [3.51;4.62] & 4.47 [3.90;5.00] & 4.19 [3.78;4.47] & 4.52 [4.12;4.89] & 4.71 [4.34;5.18] & 4.69 [4.23;5.00] & 4.40 [3.58;5.00] & 4.58 [4.40;4.81] & 4.40 [3.68;5.00] & 4.25 [3.18;4.82] \\
HGB (g/L), (median [IQR]) & 118 [98.0;136] & 145 [133;155] & 130 [114;143] & 138 [123;152] & 130 [122;143] & 142 [128;154] & 143 [128;153] & 141 [130;150] & 137 [120;152] & 140 [135;146] & 135 [120;150] & 132 [115;147] \\
PLT (109/L), (median [IQR]) & 91.0 [53.0;136] & 153 [110;201] & 157 [118;217] & 157 [111;221] & 129 [81.5;174] & 156 [119;196] & 184 [134;223] & 153 [118;220] & 159 [98.5;206] & 222 [161;238] & 154 [106;227] & 148 [98.2;210] \\
ALT (U/L), (median [IQR]) & 33.4 [22.2;137] & 25.0 [17.0;38.0] & 25.5 [18.8;38.5] & 35.0 [22.9;53.0] & 28.0 [19.4;47.0] & 30.0 [21.0;44.0] & 29.0 [21.0;40.0] & 30.8 [22.8;38.9] & 37.4 [24.0;51.4] & 29.5 [25.2;35.5] & 30.0 [16.9;43.8] & 32.2 [19.5;47.2] \\
AST (U/L), (median [IQR]) & 47.0 [31.0;448] & 26.0 [20.0;37.0] & 30.0 [22.0;40.0] & 42.1 [29.0;69.9] & 34.0 [25.4;54.8] & 34.0 [26.0;48.8] & 28.0 [22.0;37.4] & 31.9 [27.5;42.9] & 47.0 [31.5;70.7] & 27.5 [22.2;45.8] & 38.8 [27.9;67.6] & 44.9 [30.6;69.2] \\
TBIL (\mummol/L), (median [IQR]) & 32.9 [16.6;61.1] & 13.9 [10.3;18.7] & 15.5 [11.6;22.3] & 17.6 [12.7;24.4] & 18.2 [14.1;24.4] & 15.2 [11.6;20.4] & 13.0 [9.60;16.4] & 14.4 [12.3;18.9] & 18.9 [15.0;31.5] & 11.8 [8.08;14.9] & 16.2 [11.0;21.9] & 17.9 [10.9;28.1] \\
DBIL (umol/L), (median [IQR]) & 15.7 [7.40;42.3] & 5.50 [4.12;7.60] & 3.50 [2.70;5.00] & 6.80 [4.70;10.1] & 6.40 [4.40;10.6] & 3.05 [2.22;4.40] & 4.63 [3.70;6.04] & 2.75 [2.22;3.40] & 8.25 [5.65;17.5] & 3.95 [3.35;4.95] & 7.25 [4.38;12.2] & 6.90 [4.88;12.1] \\
ALB (g/L), (median [IQR]) & 35.8 [31.8;39.4] & 42.6 [39.8;45.4] & 37.8 [34.6;42.0] & 38.3 [35.3;42.0] & 39.0 [35.4;42.5] & 41.1 [38.7;43.6] & 42.0 [39.5;44.8] & 42.0 [39.4;45.0] & 37.8 [34.6;40.9] & 39.8 [37.6;41.7] & 40.6 [35.7;44.1] & 38.8 [35.0;43.2] \\
GGT (U/L), (median [IQR]) & 61.5 [34.0;131] & 44.0 [26.0;78.0] & 61.0 [33.2;90.8] & 96.7 [48.9;183] & 58.0 [31.0;113] & 51.5 [27.0;105] & 38.0 [26.0;79.0] & 43.0 [27.8;97.3] & 107 [56.6;211] & 79.0 [42.5;139] & 97.5 [39.7;199] & 95.7 [50.0;190] \\
ALP (U/L), (median [IQR]) & 103 [79.8;142] & 85.0 [69.0;108] & 98.0 [76.0;130] & 111 [84.2;159] & 98.5 [75.1;141] & 96.0 [78.0;127] & 73.0 [60.0;94.0] & 94.2 [78.8;115] & 135 [93.3;229] & 86.5 [62.8;118] & 115 [91.5;182] & 118 [80.9;199] \\
Cre (\mumol/L), (median [IQR]) & 66.0 [54.4;79.6] & 69.0 [60.0;78.0] & 67.2 [59.7;78.8] & 67.0 [58.0;75.8] & 63.3 [56.5;72.2] & 71.3 [62.1;80.2] & 81.0 [69.0;92.0] & 74.3 [66.5;79.9] & 59.3 [51.8;71.6] & 74.5 [71.0;82.0] & 60.2 [51.3;69.7] & 65.4 [54.9;74.5] \\
BUN (mmol/L), (median [IQR]) & 5.20 [4.18;6.80] & 5.20 [4.30;6.20] & 4.87 [4.11;5.89] & 4.60 [3.60;5.70] & 4.70 [3.82;5.70] & 5.38 [4.38;6.39] & 4.98 [4.13;5.70] & 5.40 [4.50;6.90] & 4.90 [3.58;5.82] & 4.26 [3.28;5.08] & 5.15 [3.72;6.03] & 4.80 [4.05;5.90] \\
UA (\mumol/L), (median [IQR]) & 302 [230;394] & 306 [256;361] & 308 [248;395] & 310 [252;376] & 260 [207;337] & 323 [276;375] & 316 [283;352] & 325 [264;390] & 298 [219;336] & 326 [300;394] & 302 [249;336] & 287 [231;352] \\
GLU (mmol/L), (median [IQR]) & 6.97 [5.12;10.0] & 5.26 [4.77;6.14] & 5.22 [4.70;6.49] & 5.40 [4.80;6.29] & 5.38 [4.80;6.16] & 5.58 [4.99;6.44] & 5.08 [4.90;5.72] & 5.43 [4.98;6.17] & 5.45 [4.90;6.50] & 5.64 [4.82;6.39] & 5.55 [5.00;6.43] & 5.60 [4.90;6.50] \\
PT (s), (median [IQR]) & 15.2 [13.1;19.1] & 11.9 [11.3;12.5] & 12.4 [11.6;13.7] & 13.1 [12.2;14.0] & 12.0 [11.3;13.0] & 13.2 [12.8;13.8] & 12.4 [11.8;13.1] & 11.8 [11.4;12.1] & 13.0 [12.0;13.9] & 11.7 [11.2;12.0] & 12.6 [11.8;13.9] & 12.9 [12.1;13.6] \\
INR, (median [IQR]) & 1.31 [1.13;1.68] & 1.03 [0.98;1.09] & 1.15 [1.06;1.27] & 1.04 [1.00;1.10] & 1.10 [1.04;1.19] & 1.02 [0.97;1.07] & 1.01 [0.96;1.06] & 1.04 [1.00;1.07] & 1.10 [1.00;1.20] & 1.00 [0.98;1.05] & 1.10 [1.00;1.20] & 1.10 [1.00;1.20] \\
APTT (s), (median [IQR]) & 31.9 [28.5;42.2] & 26.8 [24.9;29.3] & 32.6 [30.1;34.7] & 33.7 [28.2;37.7] & 33.8 [31.7;36.9] & 35.0 [32.9;37.9] & 32.3 [29.8;34.8] & 26.9 [26.0;28.3] & 28.6 [27.0;31.0] & 32.0 [29.8;34.0] & 27.7 [26.6;30.9] & 28.9 [27.1;30.9] \\
Fib (g/L), (median [IQR]) & 1.89 [1.30;2.57] & 2.55 [2.18;3.08] & 328 [258;404] & 3.30 [2.69;4.10] & 2.65 [2.28;3.33] & 2.96 [2.42;3.56] & 2.81 [2.39;3.41] & 2.53 [2.20;3.01] & 3.55 [2.77;4.60] & 3.33 [2.68;3.81] & 3.55 [2.90;5.10] & 3.80 [2.90;4.95] \\
AFP, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=400 & 294 (77.4\%) & 1569 (83.1\%) & 52 (88.1\%) & 248 (43.4\%) & 115 (86.5\%) & 234 (75.0\%) & 199 (79.9\%) & 35 (76.1\%) & 33 (43.4\%) & 16 (88.9\%) & 26 (46.4\%) & 18 (32.1\%) \\
>400 & 86 (22.6\%) & 319 (16.9\%) & 7 (11.9\%) & 324 (56.6\%) & 18 (13.5\%) & 78 (25.0\%) & 50 (20.1\%) & 11 (23.9\%) & 43 (56.6\%) & 2 (11.1\%) & 30 (53.6\%) & 38 (67.9\%) \\
PIVKA-II, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=1000 & 282 (76.0\%) & 824 (86.5\%) & 8 (61.5\%) & 252 (46.6\%) & 0 (.\%) & 134 (79.8\%) & 15 (75.0\%) & 32 (72.7\%) & 40 (52.6\%) & 12 (66.7\%) & 29 (51.8\%) & 28 (50.0\%) \\
>1000 & 89 (24.0\%) & 129 (13.5\%) & 5 (38.5\%) & 289 (53.4\%) & 0 (.\%) & 34 (20.2\%) & 5 (25.0\%) & 12 (27.3\%) & 36 (47.4\%) & 6 (33.3\%) & 27 (48.2\%) & 28 (50.0\%) \\
Tumor numbers, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
1 & 227 (55.4\%) & 1461 (75.3\%) & 46 (75.4\%) & 418 (52.3\%) & 100 (70.4\%) & 266 (85.0\%) & 236 (94.8\%) & 42 (89.4\%) & 3 (3.95\%) & 13 (72.2\%) & 2 (3.57\%) & 7 (12.5\%) \\
2 & 75 (18.3\%) & 311 (16.0\%) & 10 (16.4\%) & 90 (11.3\%) & 13 (9.15\%) & 24 (7.67\%) & 11 (4.42\%) & 3 (6.38\%) & 13 (17.1\%) & 5 (27.8\%) & 3 (5.36\%) & 7 (12.5\%) \\
3 & 34 (8.29\%) & 67 (3.45\%) & 1 (1.64\%) & 55 (6.88\%) & 2 (1.41\%) & 5 (1.60\%) & 2 (0.80\%) & 0 (0.00\%) & 5 (6.58\%) & 0 (0.00\%) & 9 (16.1\%) & 3 (5.36\%) \\
>=4 & 74 (18.0\%) & 101 (5.21\%) & 4 (6.56\%) & 236 (29.5\%) & 27 (19.0\%) & 18 (5.75\%) & 0 (0.00\%) & 2 (4.26\%) & 55 (72.4\%) & 0 (0.00\%) & 42 (75.0\%) & 39 (69.6\%) \\
Tumor maximum diameter, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=3 & 167 (40.8\%) & 1011 (52.1\%) & 11 (18.0\%) & 138 (16.9\%) & 33 (23.9\%) & 118 (37.6\%) & 97 (39.0\%) & 9 (19.1\%) & 3 (3.95\%) & 6 (33.3\%) & 3 (5.36\%) & 6 (10.7\%) \\
>3, <=5 & 98 (24.0\%) & 526 (27.1\%) & 15 (24.6\%) & 98 (12.0\%) & 35 (25.4\%) & 91 (29.0\%) & 67 (26.9\%) & 16 (34.0\%) & 3 (3.95\%) & 4 (22.2\%) & 5 (8.93\%) & 0 (0.00\%) \\
>5 & 144 (35.2\%) & 403 (20.8\%) & 35 (57.4\%) & 580 (71.1\%) & 70 (50.7\%) & 105 (33.4\%) & 85 (34.1\%) & 22 (46.8\%) & 70 (92.1\%) & 8 (44.4\%) & 48 (85.7\%) & 50 (89.3\%) \\
Vessel invasion, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 321 (77.9\%) & 1866 (96.1\%) & 47 (77.0\%) & 436 (53.4\%) & 110 (76.9\%) & 298 (94.9\%) & 242 (97.2\%) & 30 (63.8\%) & 24 (31.6\%) & 17 (94.4\%) & 18 (32.1\%) & 16 (28.6\%) \\
Yes & 91 (22.1\%) & 75 (3.86\%) & 14 (23.0\%) & 381 (46.6\%) & 33 (23.1\%) & 16 (5.10\%) & 7 (2.81\%) & 17 (36.2\%) & 52 (68.4\%) & 1 (5.56\%) & 38 (67.9\%) & 40 (71.4\%) \\
Lymph Node Metastasis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 394 (95.6\%) & 1704 (87.8\%) & 55 (90.2\%) & 756 (92.5\%) & 124 (86.7\%) & 309 (98.4\%) & 245 (98.4\%) & 47 (100\%) & 70 (92.1\%) & 18 (100\%) & 48 (85.7\%) & 49 (87.5\%) \\
Yes & 18 (4.37\%) & 237 (12.2\%) & 6 (9.84\%) & 61 (7.47\%) & 19 (13.3\%) & 5 (1.59\%) & 4 (1.61\%) & 0 (0.00\%) & 6 (7.89\%) & 0 (0.00\%) & 8 (14.3\%) & 7 (12.5\%) \\
Distant Metastasis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 397 (96.4\%) & 1890 (97.4\%) & 58 (95.1\%) & 712 (87.1\%) & 128 (89.5\%) & 312 (99.4\%) & 249 (100\%) & 47 (100\%) & 62 (81.6\%) & 17 (94.4\%) & 35 (62.5\%) & 45 (80.4\%) \\
Yes & 15 (3.64\%) & 51 (2.63\%) & 3 (4.92\%) & 105 (12.9\%) & 15 (10.5\%) & 2 (0.64\%) & 0 (0.00\%) & 0 (0.00\%) & 14 (18.4\%) & 1 (5.56\%) & 21 (37.5\%) & 11 (19.6\%) \\
BCLC stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
0 & 47 (11.4\%) & 350 (18.0\%) & 4 (6.56\%) & 29 (3.55\%) & 9 (6.29\%) & 58 (18.5\%) & 37 (14.9\%) & 3 (6.38\%) & 0 (0.00\%) & 4 (22.2\%) & 0 (0.00\%) & 0 (0.00\%) \\
A & 150 (36.4\%) & 1049 (54.0\%) & 27 (44.3\%) & 258 (31.6\%) & 62 (43.4\%) & 198 (63.1\%) & 194 (77.9\%) & 26 (55.3\%) & 0 (0.00\%) & 8 (44.4\%) & 0 (0.00\%) & 0 (0.00\%) \\
B & 73 (17.7\%) & 219 (11.3\%) & 8 (13.1\%) & 122 (14.9\%) & 18 (12.6\%) & 34 (10.8\%) & 8 (3.21\%) & 1 (2.13\%) & 23 (30.3\%) & 4 (22.2\%) & 16 (28.6\%) & 15 (26.8\%) \\
C & 94 (22.8\%) & 323 (16.6\%) & 19 (31.1\%) & 408 (49.9\%) & 54 (37.8\%) & 21 (6.69\%) & 10 (4.02\%) & 17 (36.2\%) & 53 (69.7\%) & 2 (11.1\%) & 40 (71.4\%) & 41 (73.2\%) \\
D & 48 (11.7\%) & 0 (0.00\%) & 3 (4.92\%) & 0 (0.00\%) & 0 (0.00\%) & 3 (0.96\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
CNLC stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
Ia & 126 (30.6\%) & 1036 (53.4\%) & 16 (26.2\%) & 127 (15.5\%) & 45 (31.5\%) & 179 (57.0\%) & 149 (59.8\%) & 16 (34.0\%) & 0 (0.00\%) & 9 (50.0\%) & 0 (0.00\%) & 0 (0.00\%) \\
Ib & 71 (17.2\%) & 363 (18.7\%) & 15 (24.6\%) & 160 (19.6\%) & 26 (18.2\%) & 77 (24.5\%) & 82 (32.9\%) & 13 (27.7\%) & 0 (0.00\%) & 3 (16.7\%) & 0 (0.00\%) & 0 (0.00\%) \\
IIa & 38 (9.22\%) & 162 (8.35\%) & 7 (11.5\%) & 54 (6.61\%) & 11 (7.69\%) & 19 (6.05\%) & 8 (3.21\%) & 1 (2.13\%) & 0 (0.00\%) & 4 (22.2\%) & 0 (0.00\%) & 0 (0.00\%) \\
IIb & 35 (8.50\%) & 57 (2.94\%) & 1 (1.64\%) & 68 (8.32\%) & 7 (4.90\%) & 15 (4.78\%) & 0 (0.00\%) & 0 (0.00\%) & 23 (30.3\%) & 0 (0.00\%) & 16 (28.6\%) & 15 (26.8\%) \\
IIIa & 71 (17.2\%) & 48 (2.47\%) & 12 (19.7\%) & 272 (33.3\%) & 21 (14.7\%) & 14 (4.46\%) & 6 (2.41\%) & 17 (36.2\%) & 36 (47.4\%) & 1 (5.56\%) & 16 (28.6\%) & 28 (50.0\%) \\
IIIb & 23 (5.58\%) & 275 (14.2\%) & 7 (11.5\%) & 136 (16.6\%) & 33 (23.1\%) & 7 (2.23\%) & 4 (1.61\%) & 0 (0.00\%) & 17 (22.4\%) & 1 (5.56\%) & 24 (42.9\%) & 13 (23.2\%) \\
IV & 48 (11.7\%) & 0 (0.00\%) & 3 (4.92\%) & 0 (0.00\%) & 0 (0.00\%) & 3 (0.96\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
TNM stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
IA & 54 (13.1\%) & 350 (18.0\%) & 4 (6.56\%) & 29 (3.55\%) & 9 (6.29\%) & 59 (18.8\%) & 37 (14.9\%) & 3 (6.38\%) & 0 (0.00\%) & 4 (22.2\%) & 0 (0.00\%) & 0 (0.00\%) \\
IB & 126 (30.6\%) & 899 (46.3\%) & 29 (47.5\%) & 238 (29.1\%) & 60 (42.0\%) & 192 (61.1\%) & 189 (75.9\%) & 26 (55.3\%) & 0 (0.00\%) & 8 (44.4\%) & 0 (0.00\%) & 0 (0.00\%) \\
II & 94 (22.8\%) & 280 (14.4\%) & 4 (6.56\%) & 59 (7.22\%) & 9 (6.29\%) & 25 (7.96\%) & 11 (4.42\%) & 1 (2.13\%) & 2 (2.63\%) & 1 (5.56\%) & 1 (1.79\%) & 4 (7.14\%) \\
IIIA & 31 (7.52\%) & 89 (4.59\%) & 5 (8.20\%) & 83 (10.2\%) & 11 (7.69\%) & 17 (5.41\%) & 2 (0.80\%) & 0 (0.00\%) & 21 (27.6\%) & 3 (16.7\%) & 15 (26.8\%) & 11 (19.6\%) \\
IIIB & 83 (20.1\%) & 48 (2.47\%) & 12 (19.7\%) & 272 (33.3\%) & 21 (14.7\%) & 14 (4.46\%) & 6 (2.41\%) & 17 (36.2\%) & 36 (47.4\%) & 1 (5.56\%) & 16 (28.6\%) & 28 (50.0\%) \\
IVA & 9 (2.18\%) & 224 (11.5\%) & 4 (6.56\%) & 31 (3.79\%) & 18 (12.6\%) & 5 (1.59\%) & 4 (1.61\%) & 0 (0.00\%) & 3 (3.95\%) & 0 (0.00\%) & 3 (5.36\%) & 2 (3.57\%) \\
IVB & 15 (3.64\%) & 51 (2.63\%) & 3 (4.92\%) & 105 (12.9\%) & 15 (10.5\%) & 2 (0.64\%) & 0 (0.00\%) & 0 (0.00\%) & 14 (18.4\%) & 1 (5.56\%) & 21 (37.5\%) & 11 (19.6\%) \\
Surgery, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 54 (13.1\%) & 840 (43.3\%) & 0 (0.00\%) & 317 (38.8\%) & 116 (81.1\%) & 28 (8.92\%) & 0 (0.00\%) & 0 (0.00\%) & 76 (100\%) & 0 (0.00\%) & 56 (100\%) & 56 (100\%) \\
Yes & 358 (86.9\%) & 1101 (56.7\%) & 61 (100\%) & 500 (61.2\%) & 27 (18.9\%) & 286 (91.1\%) & 249 (100\%) & 47 (100\%) & 0 (0.00\%) & 18 (100\%) & 0 (0.00\%) & 0 (0.00\%) \\
RFA, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 341 (82.8\%) & 1168 (60.2\%) & 57 (93.4\%) & 817 (100\%) & 143 (100\%) & 298 (94.9\%) & 249 (100\%) & 30 (63.8\%) & 76 (100\%) & 18 (100\%) & 56 (100\%) & 56 (100\%) \\
Yes & 71 (17.2\%) & 773 (39.8\%) & 4 (6.56\%) & 0 (0.00\%) & 0 (0.00\%) & 16 (5.10\%) & 0 (0.00\%) & 17 (36.2\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
TACE, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 224 (54.4\%) & 1870 (96.3\%) & 60 (98.4\%) & 633 (77.5\%) & 27 (18.9\%) & 299 (95.2\%) & 249 (100\%) & 45 (95.7\%) & 30 (39.5\%) & 15 (83.3\%) & 22 (39.3\%) & 22 (39.3\%) \\
Yes & 188 (45.6\%) & 71 (3.66\%) & 1 (1.64\%) & 184 (22.5\%) & 116 (81.1\%) & 15 (4.78\%) & 0 (0.00\%) & 2 (4.26\%) & 46 (60.5\%) & 3 (16.7\%) & 34 (60.7\%) & 34 (60.7\%) \\
HAIC, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 364 (88.3\%) & 1899 (97.8\%) & 61 (100\%) & 792 (96.9\%) & 143 (100\%) & 313 (99.7\%) & 249 (100\%) & 47 (100\%) & 76 (100\%) & 15 (83.3\%) & 56 (100\%) & 42 (75.0\%) \\
Yes & 48 (11.7\%) & 42 (2.16\%) & 0 (0.00\%) & 25 (3.06\%) & 0 (0.00\%) & 1 (0.32\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 3 (16.7\%) & 0 (0.00\%) & 14 (25.0\%) \\
EBRT, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 365 (88.6\%) & 1941 (100\%) & 61 (100\%) & 500 (61.2\%) & 143 (100\%) & 314 (100\%) & 249 (100\%) & 47 (100\%) & 0 (0.00\%) & 18 (100\%) & 0 (0.00\%) & 0 (0.00\%) \\
Yes & 47 (11.4\%) & 0 (0.00\%) & 0 (0.00\%) & 317 (38.8\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 76 (100\%) & 0 (0.00\%) & 56 (100\%) & 56 (100\%) \\
SIRT, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 379 (92.0\%) & 1941 (100\%) & 61 (100\%) & 817 (100\%) & 143 (100\%) & 314 (100\%) & 249 (100\%) & 47 (100\%) & 76 (100\%) & 18 (100\%) & 56 (100\%) & 56 (100\%) \\
Yes & 33 (8.01\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
TKI, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 284 (68.9\%) & 1861 (95.9\%) & 53 (86.9\%) & 536 (65.6\%) & 42 (29.4\%) & 292 (93.0\%) & 238 (95.6\%) & 19 (40.4\%) & 10 (13.2\%) & 14 (77.8\%) & 8 (14.3\%) & 6 (10.7\%) \\
Yes & 128 (31.1\%) & 80 (4.12\%) & 8 (13.1\%) & 281 (34.4\%) & 101 (70.6\%) & 22 (7.01\%) & 11 (4.42\%) & 28 (59.6\%) & 66 (86.8\%) & 4 (22.2\%) & 48 (85.7\%) & 50 (89.3\%) \\
ICIs, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 318 (77.2\%) & 1851 (95.4\%) & 60 (98.4\%) & 548 (67.1\%) & 39 (27.3\%) & 256 (81.5\%) & 238 (95.6\%) & 16 (34.0\%) & 14 (18.4\%) & 14 (77.8\%) & 12 (21.4\%) & 12 (21.4\%) \\
Yes & 94 (22.8\%) & 90 (4.64\%) & 1 (1.64\%) & 269 (32.9\%) & 104 (72.7\%) & 58 (18.5\%) & 11 (4.42\%) & 31 (66.0\%) & 62 (81.6\%) & 4 (22.2\%) & 44 (78.6\%) & 44 (78.6\%) \\

    \end{longtable}
    \end{center}
    \end{landscape}


==> baseline_full_external.tex <==
    % Preamble needed:
    % \usepackage{pdflscape,longtable,booktabs,array}
    % \usepackage{caption} % optional for caption*
    % Example usage: place this entire environment where you want the table.
    \begin{landscape}
    \begin{center}
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.25}
    \begin{longtable}{p{5.2cm}p{3.0cm}}}}}}}}}}}}}
    \caption{Baseline characteristics of patients in the external multi-center HCC cohort (full dataset)}\label{tab:baseline_full_external}\\
\toprule
Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
\midrule
\endfirsthead
\caption*{Baseline characteristics of patients in the external multi-center HCC cohort (full dataset) (continued)}\\
\toprule
Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
\midrule
\endhead
\midrule
\multicolumn{13}{r}{\small Continued on next page}\\
\bottomrule
\endfoot
\bottomrule
\endlastfoot

     & (N=1398) & (N=1994) & (N=945) & (N=865) & (N=431) & (N=319) & (N=299) & (N=165) & (N=76) & (N=63) & (N=57) & (N=56) \\
Sex, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
female & 260 (18.6\%) & 406 (20.4\%) & 213 (22.5\%) & 109 (12.6\%) & 93 (21.6\%) & 55 (17.2\%) & 47 (15.7\%) & 29 (17.6\%) & 10 (13.2\%) & 9 (14.3\%) & 9 (15.8\%) & 8 (14.3\%) \\
male & 1138 (81.4\%) & 1588 (79.6\%) & 732 (77.5\%) & 756 (87.4\%) & 338 (78.4\%) & 264 (82.8\%) & 252 (84.3\%) & 136 (82.4\%) & 66 (86.8\%) & 54 (85.7\%) & 48 (84.2\%) & 48 (85.7\%) \\
Age (years), (median [IQR]) & 59.0 [51.0;66.0] & 60.0 [53.0;66.0] & 59.0 [50.0;66.0] & 57.0 [48.0;64.0] & 61.0 [53.0;67.0] & 61.0 [53.0;68.0] & 56.0 [47.0;65.0] & 52.0 [46.0;60.0] & 61.0 [51.0;69.0] & 54.0 [45.0;62.0] & 60.0 [52.0;65.0] & 54.5 [45.8;65.2] \\
BMI (kg/m2), (median [IQR]) & 23.8 [21.5;25.8] & 24.2 [22.3;26.8] & 22.8 [20.8;24.8] & 23.7 [21.7;26.3] & 23.6 [21.4;26.0] & 23.5 [20.4;26.7] & 23.5 [21.3;25.6] & 23.4 [21.3;25.6] & 23.9 [22.4;26.1] & 23.5 [20.8;25.4] & 23.7 [21.2;26.8] & 24.3 [20.4;26.0] \\
Diabetes, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 727 (73.7\%) & 1603 (80.4\%) & 696 (85.1\%) & 682 (82.8\%) & 286 (88.5\%) & 254 (79.6\%) & 252 (84.3\%) & 136 (82.4\%) & 57 (75.0\%) & 56 (88.9\%) & 40 (70.2\%) & 51 (91.1\%) \\
Yes & 260 (26.3\%) & 391 (19.6\%) & 122 (14.9\%) & 142 (17.2\%) & 37 (11.5\%) & 65 (20.4\%) & 47 (15.7\%) & 29 (17.6\%) & 19 (25.0\%) & 7 (11.1\%) & 17 (29.8\%) & 5 (8.93\%) \\
Hypertension, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 660 (66.9\%) & 1302 (65.3\%) & 586 (77.4\%) & 663 (80.5\%) & 294 (74.8\%) & 205 (64.3\%) & 237 (79.3\%) & 138 (83.6\%) & 53 (69.7\%) & 53 (84.1\%) & 42 (73.7\%) & 43 (76.8\%) \\
Yes & 326 (33.1\%) & 692 (34.7\%) & 171 (22.6\%) & 161 (19.5\%) & 99 (25.2\%) & 114 (35.7\%) & 62 (20.7\%) & 27 (16.4\%) & 23 (30.3\%) & 10 (15.9\%) & 15 (26.3\%) & 13 (23.2\%) \\
Cirrhosis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 412 (40.9\%) & 444 (22.3\%) & 363 (46.4\%) & 429 (56.1\%) & 39 (9.90\%) & 138 (43.3\%) & 122 (40.8\%) & 59 (35.8\%) & 9 (11.8\%) & 18 (28.6\%) & 15 (26.3\%) & 7 (12.5\%) \\
Yes & 596 (59.1\%) & 1543 (77.7\%) & 420 (53.6\%) & 336 (43.9\%) & 355 (90.1\%) & 181 (56.7\%) & 177 (59.2\%) & 106 (64.2\%) & 67 (88.2\%) & 45 (71.4\%) & 42 (73.7\%) & 49 (87.5\%) \\
Chronic liver disease, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 182 (15.9\%) & 192 (9.63\%) & 47 (6.83\%) & 124 (15.0\%) & 30 (7.46\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 1 (1.59\%) & 0 (0.00\%) & 0 (0.00\%) \\
HBV & 850 (74.4\%) & 1471 (73.8\%) & 476 (69.2\%) & 626 (76.0\%) & 353 (87.8\%) & 237 (74.3\%) & 250 (83.6\%) & 144 (87.3\%) & 65 (85.5\%) & 56 (88.9\%) & 49 (86.0\%) & 47 (83.9\%) \\
HBV+HCV & 6 (0.53\%) & 12 (0.60\%) & 0 (0.00\%) & 8 (0.97\%) & 0 (0.00\%) & 2 (0.63\%) & 1 (0.33\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
HCV & 24 (2.10\%) & 140 (7.02\%) & 15 (2.18\%) & 22 (2.67\%) & 7 (1.74\%) & 0 (0.00\%) & 8 (2.68\%) & 2 (1.21\%) & 4 (5.26\%) & 1 (1.59\%) & 6 (10.5\%) & 2 (3.57\%) \\
Others & 80 (7.01\%) & 179 (8.98\%) & 150 (21.8\%) & 44 (5.34\%) & 12 (2.99\%) & 80 (25.1\%) & 40 (13.4\%) & 19 (11.5\%) & 7 (9.21\%) & 5 (7.94\%) & 2 (3.51\%) & 7 (12.5\%) \\
ECOG PS, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
0 & 669 (54.9\%) & 1228 (61.6\%) & 248 (34.4\%) & 467 (55.5\%) & 144 (61.3\%) & 319 (100\%) & 66 (23.5\%) & 67 (40.6\%) & 38 (50.0\%) & 21 (33.9\%) & 30 (52.6\%) & 27 (48.2\%) \\
1 & 433 (35.6\%) & 766 (38.4\%) & 353 (49.0\%) & 328 (39.0\%) & 70 (29.8\%) & 0 (0.00\%) & 197 (70.1\%) & 97 (58.8\%) & 38 (50.0\%) & 35 (56.5\%) & 19 (33.3\%) & 24 (42.9\%) \\
2 & 110 (9.03\%) & 0 (0.00\%) & 113 (15.7\%) & 47 (5.58\%) & 21 (8.94\%) & 0 (0.00\%) & 18 (6.41\%) & 1 (0.61\%) & 0 (0.00\%) & 5 (8.06\%) & 8 (14.0\%) & 5 (8.93\%) \\
3 & 6 (0.49\%) & 0 (0.00\%) & 5 (0.69\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 1 (1.61\%) & 0 (0.00\%) & 0 (0.00\%) \\
4 & 0 (0.00\%) & 0 (0.00\%) & 1 (0.14\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
Child-Pugh stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
A & 810 (69.4\%) & 1752 (88.0\%) & 703 (85.1\%) & 627 (74.5\%) & 314 (79.7\%) & 303 (95.0\%) & 293 (98.0\%) & 164 (99.4\%) & 59 (77.6\%) & 59 (93.7\%) & 47 (82.5\%) & 49 (87.5\%) \\
B & 307 (26.3\%) & 239 (12.0\%) & 117 (14.2\%) & 215 (25.5\%) & 78 (19.8\%) & 13 (4.08\%) & 6 (2.01\%) & 1 (0.61\%) & 17 (22.4\%) & 4 (6.35\%) & 10 (17.5\%) & 7 (12.5\%) \\
C & 50 (4.28\%) & 0 (0.00\%) & 6 (0.73\%) & 0 (0.00\%) & 2 (0.51\%) & 3 (0.94\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
mALBI\_stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
Grade 1 & 363 (33.2\%) & 1498 (76.0\%) & 331 (38.3\%) & 289 (39.5\%) & 145 (34.4\%) & 210 (65.8\%) & 225 (75.3\%) & 126 (76.4\%) & 26 (34.2\%) & 36 (57.1\%) & 32 (56.1\%) & 26 (46.4\%) \\
Grade 2a & 274 (25.0\%) & 292 (14.8\%) & 204 (23.6\%) & 202 (27.6\%) & 96 (22.8\%) & 72 (22.6\%) & 50 (16.7\%) & 27 (16.4\%) & 15 (19.7\%) & 16 (25.4\%) & 6 (10.5\%) & 10 (17.9\%) \\
Grade 2b & 392 (35.8\%) & 172 (8.73\%) & 238 (27.5\%) & 220 (30.1\%) & 171 (40.6\%) & 35 (11.0\%) & 23 (7.69\%) & 11 (6.67\%) & 29 (38.2\%) & 10 (15.9\%) & 17 (29.8\%) & 19 (33.9\%) \\
Grade 3 & 66 (6.03\%) & 8 (0.41\%) & 92 (10.6\%) & 21 (2.87\%) & 9 (2.14\%) & 2 (0.63\%) & 1 (0.33\%) & 1 (0.61\%) & 6 (7.89\%) & 1 (1.59\%) & 2 (3.51\%) & 1 (1.79\%) \\
WBC (109/L), (median [IQR]) & 4.69 [3.47;6.26] & 5.11 [4.08;6.29] & 5.38 [4.20;7.40] & 5.50 [4.10;7.17] & 5.00 [3.80;6.30] & 5.60 [4.50;7.00] & 5.56 [4.50;7.04] & 5.18 [4.29;6.57] & 4.80 [3.88;6.15] & 6.26 [5.30;7.62] & 5.20 [3.40;6.40] & 4.55 [3.10;5.85] \\
NEUT (109/L), (median [IQR]) & 3.06 [2.12;4.50] & 2.86 [2.15;3.74] & 3.50 [2.40;5.68] & 3.40 [2.40;4.80] & 2.90 [2.16;4.10] & 3.57 [2.66;4.64] & 3.00 [2.40;4.15] & 3.24 [2.51;4.08] & 3.15 [2.40;4.60] & 3.89 [3.12;5.14] & 3.70 [2.50;4.70] & 3.25 [2.28;4.50] \\
LYMPH (109/L), (median [IQR]) & 1.01 [0.61;1.46] & 1.54 [1.19;1.96] & 1.17 [0.80;1.50] & 1.28 [0.88;1.74] & 1.30 [0.90;1.70] & 1.48 [1.07;1.85] & 1.68 [1.31;2.09] & 1.35 [1.02;1.71] & 0.90 [0.70;1.40] & 1.67 [1.30;2.03] & 1.10 [0.70;1.50] & 0.85 [0.60;1.20] \\
RBC (1012/L), (median [IQR]) & 4.03 [3.48;4.51] & 4.62 [4.23;4.98] & 4.09 [3.66;4.56] & 4.48 [3.92;5.00] & 4.06 [3.59;4.45] & 4.52 [4.12;4.88] & 4.70 [4.34;5.18] & 4.76 [4.40;5.11] & 4.40 [3.58;5.00] & 4.59 [4.25;4.86] & 4.40 [3.60;5.00] & 4.25 [3.18;4.82] \\
HGB (g/L), (median [IQR]) & 126 [110;139] & 145 [133;155] & 131 [116;142] & 138 [123;152] & 130 [118;143] & 142 [128;154] & 144 [128;154] & 146 [133;156] & 137 [120;152] & 139 [126;145] & 135 [120;150] & 132 [115;147] \\
PLT (109/L), (median [IQR]) & 135 [86.2;191] & 153 [110;200] & 154 [113;205] & 158 [111;222] & 124 [79.8;177] & 156 [118;196] & 184 [132;227] & 160 [123;216] & 159 [98.5;206] & 220 [158;282] & 152 [104;227] & 148 [98.2;210] \\
ALT (U/L), (median [IQR]) & 27.7 [17.6;47.4] & 25.0 [17.0;38.0] & 28.0 [18.0;47.0] & 35.0 [22.9;53.0] & 30.8 [21.0;45.7] & 30.0 [21.0;44.0] & 29.0 [22.0;41.0] & 30.1 [22.2;43.9] & 37.4 [24.0;51.4] & 31.0 [25.5;50.5] & 30.0 [15.8;43.1] & 32.2 [19.5;47.2] \\
AST (U/L), (median [IQR]) & 39.3 [25.0;78.3] & 26.0 [20.0;37.0] & 31.0 [22.0;46.0] & 42.0 [29.4;68.9] & 35.6 [25.0;54.8] & 34.0 [25.5;49.0] & 28.0 [22.0;40.0] & 31.9 [26.2;41.8] & 47.0 [31.5;70.7] & 42.0 [26.0;60.5] & 37.2 [27.4;67.0] & 44.9 [30.6;69.2] \\
TBIL (\mummol/L), (median [IQR]) & 15.3 [10.3;27.6] & 14.0 [10.3;18.7] & 15.6 [11.6;21.2] & 17.5 [12.7;24.1] & 18.1 [13.5;25.5] & 15.3 [11.7;20.4] & 13.3 [9.75;16.9] & 15.1 [12.1;19.6] & 18.9 [15.0;31.5] & 12.4 [8.15;18.8] & 16.2 [11.2;22.0] & 17.9 [10.9;28.1] \\
DBIL (umol/L), (median [IQR]) & 6.80 [4.60;14.2] & 5.50 [4.20;7.60] & 3.90 [2.70;6.10] & 6.70 [4.60;10.0] & 6.50 [4.40;10.1] & 3.10 [2.30;4.45] & 4.59 [3.50;6.06] & 2.83 [2.20;3.70] & 8.25 [5.65;17.5] & 4.10 [3.15;6.55] & 7.30 [4.40;12.4] & 6.90 [4.88;12.1] \\
ALB (g/L), (median [IQR]) & 37.1 [33.9;40.3] & 42.5 [39.7;45.4] & 38.3 [34.9;41.9] & 38.2 [35.3;42.0] & 37.7 [34.2;41.6] & 41.1 [38.7;43.5] & 42.2 [39.3;44.8] & 42.8 [39.8;45.8] & 37.8 [34.6;40.9] & 38.9 [36.0;41.9] & 40.6 [35.5;44.1] & 38.8 [35.0;43.2] \\
GGT (U/L), (median [IQR]) & 72.0 [37.0;162] & 44.0 [27.0;79.0] & 58.5 [31.0;121] & 96.0 [48.0;180] & 59.0 [32.0;117] & 53.0 [27.5;105] & 41.0 [27.0;80.0] & 48.3 [29.0;95.5] & 107 [56.6;211] & 106 [55.0;196] & 97.5 [39.7;198] & 95.7 [50.0;190] \\
ALP (U/L), (median [IQR]) & 102 [76.0;152] & 85.0 [69.0;108] & 97.0 [76.0;132] & 110 [84.5;160] & 106 [78.0;146] & 96.5 [78.0;128] & 74.0 [61.0;94.0] & 93.1 [77.7;111] & 135 [93.3;229] & 110 [80.0;152] & 114 [92.0;181] & 118 [80.9;199] \\
Cre (\mumol/L), (median [IQR]) & 67.0 [57.0;78.0] & 69.0 [60.0;78.0] & 67.9 [59.3;78.7] & 67.0 [58.0;76.0] & 63.5 [55.1;73.7] & 71.4 [62.2;80.2] & 81.0 [68.0;93.0] & 75.8 [68.1;83.8] & 59.3 [51.8;71.6] & 73.0 [66.0;78.0] & 60.3 [51.4;69.0] & 65.4 [54.9;74.5] \\
BUN (mmol/L), (median [IQR]) & 5.00 [3.90;6.30] & 5.20 [4.30;6.20] & 5.21 [4.20;6.36] & 4.50 [3.60;5.70] & 4.75 [3.98;5.83] & 5.38 [4.38;6.43] & 4.90 [4.11;5.68] & 5.48 [4.50;6.33] & 4.90 [3.58;5.82] & 4.49 [3.37;5.46] & 5.10 [3.80;6.00] & 4.80 [4.05;5.90] \\
UA (\mumol/L), (median [IQR]) & 308 [253;386] & 306 [256;361] & 301 [235;367] & 311 [253;376] & 271 [213;333] & 323 [276;377] & 315 [284;360] & 346 [285;406] & 298 [219;336] & 320 [268;370] & 299 [251;336] & 287 [231;352] \\
GLU (mmol/L), (median [IQR]) & 5.46 [4.87;7.26] & 5.25 [4.77;6.15] & 5.11 [4.58;6.18] & 5.38 [4.78;6.22] & 5.38 [4.84;6.20] & 5.58 [4.99;6.49] & 5.08 [4.89;5.72] & 5.28 [4.77;6.10] & 5.45 [4.90;6.50] & 5.80 [5.00;7.28] & 5.50 [5.00;6.40] & 5.60 [4.90;6.50] \\
PT (s), (median [IQR]) & 12.6 [11.9;14.2] & 11.9 [11.3;12.5] & 12.2 [11.4;13.0] & 13.1 [12.3;14.0] & 12.1 [11.3;12.9] & 13.2 [12.8;13.8] & 12.3 [11.7;13.0] & 11.7 [11.3;12.2] & 13.0 [12.0;13.9] & 11.9 [11.3;12.6] & 12.6 [11.8;13.9] & 12.9 [12.1;13.6] \\
INR, (median [IQR]) & 1.08 [1.02;1.23] & 1.03 [0.98;1.09] & 1.12 [1.04;1.19] & 1.04 [1.00;1.10] & 1.10 [1.04;1.19] & 1.02 [0.97;1.07] & 1.01 [0.96;1.06] & 1.04 [1.00;1.08] & 1.10 [1.00;1.20] & 1.05 [1.00;1.12] & 1.10 [1.00;1.20] & 1.10 [1.00;1.20] \\
APTT (s), (median [IQR]) & 28.8 [27.1;31.9] & 26.8 [24.9;29.3] & 31.3 [29.3;33.7] & 33.9 [28.5;37.7] & 34.1 [31.5;37.1] & 35.0 [33.0;37.8] & 32.3 [29.9;34.6] & 27.6 [26.2;29.0] & 28.6 [27.0;31.0] & 32.7 [30.7;34.6] & 27.7 [26.6;31.1] & 28.9 [27.1;30.9] \\
Fib (g/L), (median [IQR]) & 2.43 [1.82;3.18] & 2.55 [2.18;3.09] & 309 [248;393] & 3.30 [2.68;4.11] & 2.66 [2.21;3.25] & 2.96 [2.42;3.57] & 2.81 [2.39;3.41] & 2.53 [2.20;2.97] & 3.55 [2.77;4.60] & 3.38 [2.81;4.07] & 3.50 [2.90;5.10] & 3.80 [2.90;4.95] \\
AFP, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=400 & 827 (78.5\%) & 1608 (82.9\%) & 578 (77.4\%) & 259 (43.1\%) & 341 (85.0\%) & 238 (75.1\%) & 235 (78.6\%) & 115 (71.0\%) & 33 (43.4\%) & 37 (58.7\%) & 26 (45.6\%) & 18 (32.1\%) \\
>400 & 227 (21.5\%) & 332 (17.1\%) & 169 (22.6\%) & 342 (56.9\%) & 60 (15.0\%) & 79 (24.9\%) & 64 (21.4\%) & 47 (29.0\%) & 43 (56.6\%) & 26 (41.3\%) & 31 (54.4\%) & 38 (67.9\%) \\
PIVKA-II, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=1000 & 759 (73.6\%) & 844 (85.7\%) & 171 (65.8\%) & 258 (45.9\%) & 0 (.\%) & 135 (79.4\%) & 16 (72.7\%) & 121 (76.6\%) & 40 (52.6\%) & 34 (54.0\%) & 30 (52.6\%) & 28 (50.0\%) \\
>1000 & 272 (26.4\%) & 141 (14.3\%) & 89 (34.2\%) & 304 (54.1\%) & 0 (.\%) & 35 (20.6\%) & 6 (27.3\%) & 37 (23.4\%) & 36 (47.4\%) & 29 (46.0\%) & 27 (47.4\%) & 28 (50.0\%) \\
Tumor numbers, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
1 & 675 (57.9\%) & 1491 (75.3\%) & 529 (75.5\%) & 431 (52.5\%) & 225 (66.8\%) & 268 (84.3\%) & 284 (95.0\%) & 147 (89.1\%) & 3 (3.95\%) & 34 (54.8\%) & 2 (3.51\%) & 7 (12.5\%) \\
2 & 160 (13.7\%) & 315 (15.9\%) & 105 (15.0\%) & 93 (11.3\%) & 36 (10.7\%) & 25 (7.86\%) & 12 (4.01\%) & 7 (4.24\%) & 13 (17.1\%) & 12 (19.4\%) & 3 (5.26\%) & 7 (12.5\%) \\
3 & 85 (7.29\%) & 67 (3.38\%) & 19 (2.71\%) & 55 (6.70\%) & 6 (1.78\%) & 5 (1.57\%) & 3 (1.00\%) & 1 (0.61\%) & 5 (6.58\%) & 1 (1.61\%) & 9 (15.8\%) & 3 (5.36\%) \\
>=4 & 246 (21.1\%) & 107 (5.40\%) & 48 (6.85\%) & 242 (29.5\%) & 70 (20.8\%) & 20 (6.29\%) & 0 (0.00\%) & 10 (6.06\%) & 55 (72.4\%) & 15 (24.2\%) & 43 (75.4\%) & 39 (69.6\%) \\
Tumor maximum diameter, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
<=3 & 341 (29.8\%) & 1023 (51.7\%) & 161 (23.9\%) & 150 (17.4\%) & 90 (28.2\%) & 120 (37.7\%) & 97 (38.6\%) & 48 (29.1\%) & 3 (3.95\%) & 12 (19.4\%) & 3 (5.26\%) & 6 (10.7\%) \\
>3, <=5 & 274 (23.9\%) & 539 (27.3\%) & 174 (25.8\%) & 109 (12.6\%) & 78 (24.5\%) & 91 (28.6\%) & 67 (26.7\%) & 46 (27.9\%) & 3 (3.95\%) & 11 (17.7\%) & 6 (10.5\%) & 0 (0.00\%) \\
>5 & 531 (46.3\%) & 415 (21.0\%) & 340 (50.4\%) & 605 (70.0\%) & 151 (47.3\%) & 107 (33.6\%) & 87 (34.7\%) & 71 (43.0\%) & 70 (92.1\%) & 39 (62.9\%) & 48 (84.2\%) & 50 (89.3\%) \\
Vessel invasion, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 898 (75.7\%) & 1901 (96.0\%) & 453 (64.3\%) & 471 (54.5\%) & 182 (76.8\%) & 301 (94.4\%) & 291 (97.3\%) & 125 (75.8\%) & 24 (31.6\%) & 50 (79.4\%) & 18 (31.6\%) & 16 (28.6\%) \\
Yes & 288 (24.3\%) & 79 (3.99\%) & 252 (35.7\%) & 394 (45.5\%) & 55 (23.2\%) & 18 (5.64\%) & 8 (2.68\%) & 40 (24.2\%) & 52 (68.4\%) & 13 (20.6\%) & 39 (68.4\%) & 40 (71.4\%) \\
Lymph Node Metastasis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 879 (87.8\%) & 1738 (87.8\%) & 603 (85.9\%) & 800 (92.5\%) & 378 (87.7\%) & 314 (98.4\%) & 295 (98.7\%) & 165 (100\%) & 70 (92.1\%) & 55 (87.3\%) & 48 (84.2\%) & 49 (87.5\%) \\
Yes & 122 (12.2\%) & 241 (12.2\%) & 99 (14.1\%) & 65 (7.51\%) & 53 (12.3\%) & 5 (1.57\%) & 4 (1.34\%) & 0 (0.00\%) & 6 (7.89\%) & 8 (12.7\%) & 9 (15.8\%) & 7 (12.5\%) \\
Distant Metastasis, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 870 (86.1\%) & 1926 (97.3\%) & 636 (90.3\%) & 757 (87.5\%) & 376 (87.2\%) & 317 (99.4\%) & 299 (100\%) & 162 (99.4\%) & 62 (81.6\%) & 52 (82.5\%) & 35 (61.4\%) & 45 (80.4\%) \\
Yes & 140 (13.9\%) & 53 (2.68\%) & 68 (9.66\%) & 108 (12.5\%) & 55 (12.8\%) & 2 (0.63\%) & 0 (0.00\%) & 1 (0.61\%) & 14 (18.4\%) & 11 (17.5\%) & 22 (38.6\%) & 11 (19.6\%) \\
BCLC stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
0 & 98 (9.91\%) & 354 (17.9\%) & 36 (5.68\%) & 32 (3.80\%) & 13 (5.51\%) & 59 (18.5\%) & 37 (14.7\%) & 19 (11.7\%) & 0 (0.00\%) & 6 (9.68\%) & 0 (0.00\%) & 0 (0.00\%) \\
A & 382 (38.6\%) & 1068 (54.1\%) & 249 (39.3\%) & 264 (31.4\%) & 92 (39.0\%) & 199 (62.4\%) & 195 (77.7\%) & 95 (58.3\%) & 0 (0.00\%) & 20 (32.3\%) & 0 (0.00\%) & 0 (0.00\%) \\
B & 131 (13.2\%) & 223 (11.3\%) & 58 (9.15\%) & 123 (14.6\%) & 32 (13.6\%) & 35 (11.0\%) & 8 (3.19\%) & 9 (5.52\%) & 23 (30.3\%) & 17 (27.4\%) & 16 (28.1\%) & 15 (26.8\%) \\
C & 328 (33.2\%) & 329 (16.7\%) & 285 (45.0\%) & 423 (50.2\%) & 97 (41.1\%) & 23 (7.21\%) & 11 (4.38\%) & 40 (24.5\%) & 53 (69.7\%) & 19 (30.6\%) & 41 (71.9\%) & 41 (73.2\%) \\
D & 50 (5.06\%) & 0 (0.00\%) & 6 (0.95\%) & 0 (0.00\%) & 2 (0.85\%) & 3 (0.94\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
CNLC stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
Ia & 300 (30.2\%) & 1050 (53.2\%) & 155 (24.3\%) & 131 (15.6\%) & 64 (27.1\%) & 181 (56.7\%) & 149 (59.4\%) & 65 (39.9\%) & 0 (0.00\%) & 15 (24.2\%) & 0 (0.00\%) & 0 (0.00\%) \\
Ib & 179 (18.0\%) & 372 (18.8\%) & 128 (20.1\%) & 165 (19.6\%) & 41 (17.4\%) & 77 (24.1\%) & 83 (33.1\%) & 49 (30.1\%) & 0 (0.00\%) & 11 (17.7\%) & 0 (0.00\%) & 0 (0.00\%) \\
IIa & 80 (8.06\%) & 164 (8.31\%) & 41 (6.44\%) & 55 (6.53\%) & 14 (5.93\%) & 20 (6.27\%) & 8 (3.19\%) & 2 (1.23\%) & 0 (0.00\%) & 10 (16.1\%) & 0 (0.00\%) & 0 (0.00\%) \\
IIb & 51 (5.14\%) & 59 (2.99\%) & 16 (2.51\%) & 68 (8.08\%) & 18 (7.63\%) & 15 (4.70\%) & 0 (0.00\%) & 7 (4.29\%) & 23 (30.3\%) & 7 (11.3\%) & 16 (28.1\%) & 15 (26.8\%) \\
IIIa & 152 (15.3\%) & 50 (2.53\%) & 178 (27.9\%) & 282 (33.5\%) & 34 (14.4\%) & 16 (5.02\%) & 7 (2.79\%) & 39 (23.9\%) & 36 (47.4\%) & 6 (9.68\%) & 16 (28.1\%) & 28 (50.0\%) \\
IIIb & 175 (17.6\%) & 279 (14.1\%) & 107 (16.8\%) & 141 (16.7\%) & 63 (26.7\%) & 7 (2.19\%) & 4 (1.59\%) & 1 (0.61\%) & 17 (22.4\%) & 12 (19.4\%) & 25 (43.9\%) & 13 (23.2\%) \\
IV & 56 (5.64\%) & 0 (0.00\%) & 12 (1.88\%) & 0 (0.00\%) & 2 (0.85\%) & 3 (0.94\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 1 (1.61\%) & 0 (0.00\%) & 0 (0.00\%) \\
TNM stage, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
IA & 105 (10.7\%) & 354 (17.9\%) & 36 (5.76\%) & 32 (3.81\%) & 13 (5.78\%) & 60 (18.8\%) & 37 (14.7\%) & 19 (11.7\%) & 0 (0.00\%) & 6 (9.84\%) & 0 (0.00\%) & 0 (0.00\%) \\
IB & 339 (34.6\%) & 917 (46.5\%) & 241 (38.6\%) & 244 (29.0\%) & 86 (38.2\%) & 193 (60.5\%) & 190 (75.7\%) & 92 (56.4\%) & 0 (0.00\%) & 19 (31.1\%) & 0 (0.00\%) & 0 (0.00\%) \\
II & 138 (14.1\%) & 285 (14.4\%) & 38 (6.08\%) & 59 (7.02\%) & 20 (8.89\%) & 25 (7.84\%) & 11 (4.38\%) & 12 (7.36\%) & 2 (2.63\%) & 7 (11.5\%) & 1 (1.75\%) & 4 (7.14\%) \\
IIIA & 64 (6.54\%) & 89 (4.51\%) & 30 (4.80\%) & 84 (10.0\%) & 16 (7.11\%) & 18 (5.64\%) & 2 (0.80\%) & 0 (0.00\%) & 21 (27.6\%) & 11 (18.0\%) & 15 (26.3\%) & 11 (19.6\%) \\
IIIB & 166 (17.0\%) & 50 (2.53\%) & 178 (28.5\%) & 282 (33.6\%) & 34 (15.1\%) & 16 (5.02\%) & 7 (2.79\%) & 39 (23.9\%) & 36 (47.4\%) & 6 (9.84\%) & 16 (28.1\%) & 28 (50.0\%) \\
IVA & 51 (5.21\%) & 227 (11.5\%) & 45 (7.20\%) & 31 (3.69\%) & 29 (12.9\%) & 5 (1.57\%) & 4 (1.59\%) & 0 (0.00\%) & 3 (3.95\%) & 1 (1.64\%) & 3 (5.26\%) & 2 (3.57\%) \\
IVB & 116 (11.8\%) & 52 (2.63\%) & 57 (9.12\%) & 108 (12.9\%) & 27 (12.0\%) & 2 (0.63\%) & 0 (0.00\%) & 1 (0.61\%) & 14 (18.4\%) & 11 (18.0\%) & 22 (38.6\%) & 11 (19.6\%) \\
Surgery, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 635 (45.4\%) & 866 (43.4\%) & 309 (32.7\%) & 323 (37.3\%) & 323 (74.9\%) & 30 (9.40\%) & 0 (0.00\%) & 0 (0.00\%) & 76 (100\%) & 41 (65.1\%) & 57 (100\%) & 56 (100\%) \\
Yes & 763 (54.6\%) & 1128 (56.6\%) & 636 (67.3\%) & 542 (62.7\%) & 108 (25.1\%) & 289 (90.6\%) & 299 (100\%) & 165 (100\%) & 0 (0.00\%) & 22 (34.9\%) & 0 (0.00\%) & 0 (0.00\%) \\
RFA, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 1290 (92.3\%) & 1209 (60.6\%) & 902 (95.4\%) & 865 (100\%) & 431 (100\%) & 303 (95.0\%) & 299 (100\%) & 116 (70.3\%) & 76 (100\%) & 58 (92.1\%) & 57 (100\%) & 56 (100\%) \\
Yes & 108 (7.73\%) & 785 (39.4\%) & 43 (4.55\%) & 0 (0.00\%) & 0 (0.00\%) & 16 (5.02\%) & 0 (0.00\%) & 49 (29.7\%) & 0 (0.00\%) & 5 (7.94\%) & 0 (0.00\%) & 0 (0.00\%) \\
TACE, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 892 (63.8\%) & 1914 (96.0\%) & 863 (91.3\%) & 679 (78.5\%) & 108 (25.1\%) & 302 (94.7\%) & 299 (100\%) & 159 (96.4\%) & 30 (39.5\%) & 34 (54.0\%) & 22 (38.6\%) & 22 (39.3\%) \\
Yes & 506 (36.2\%) & 80 (4.01\%) & 82 (8.68\%) & 186 (21.5\%) & 323 (74.9\%) & 17 (5.33\%) & 0 (0.00\%) & 6 (3.64\%) & 46 (60.5\%) & 29 (46.0\%) & 35 (61.4\%) & 34 (60.7\%) \\
HAIC, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 1181 (84.5\%) & 1943 (97.4\%) & 938 (99.3\%) & 840 (97.1\%) & 431 (100\%) & 318 (99.7\%) & 299 (100\%) & 162 (98.2\%) & 76 (100\%) & 38 (60.3\%) & 57 (100\%) & 42 (75.0\%) \\
Yes & 217 (15.5\%) & 51 (2.56\%) & 7 (0.74\%) & 25 (2.89\%) & 0 (0.00\%) & 1 (0.31\%) & 0 (0.00\%) & 3 (1.82\%) & 0 (0.00\%) & 25 (39.7\%) & 0 (0.00\%) & 14 (25.0\%) \\
EBRT, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 1319 (94.3\%) & 1994 (100\%) & 945 (100\%) & 542 (62.7\%) & 431 (100\%) & 319 (100\%) & 299 (100\%) & 165 (100\%) & 0 (0.00\%) & 63 (100\%) & 0 (0.00\%) & 0 (0.00\%) \\
Yes & 79 (5.65\%) & 0 (0.00\%) & 0 (0.00\%) & 323 (37.3\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 76 (100\%) & 0 (0.00\%) & 57 (100\%) & 56 (100\%) \\
SIRT, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 976 (69.8\%) & 1994 (100\%) & 945 (100\%) & 865 (100\%) & 431 (100\%) & 319 (100\%) & 299 (100\%) & 165 (100\%) & 76 (100\%) & 63 (100\%) & 57 (100\%) & 56 (100\%) \\
Yes & 422 (30.2\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) & 0 (0.00\%) \\
TKI, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 972 (69.5\%) & 1898 (95.2\%) & 639 (67.6\%) & 578 (66.8\%) & 137 (31.8\%) & 296 (92.8\%) & 287 (96.0\%) & 99 (60.0\%) & 10 (13.2\%) & 24 (38.1\%) & 8 (14.0\%) & 6 (10.7\%) \\
Yes & 426 (30.5\%) & 96 (4.81\%) & 306 (32.4\%) & 287 (33.2\%) & 294 (68.2\%) & 23 (7.21\%) & 12 (4.01\%) & 66 (40.0\%) & 66 (86.8\%) & 39 (61.9\%) & 49 (86.0\%) & 50 (89.3\%) \\
ICIs, n (\%) &  &  &  &  &  &  &  &  &  &  &  &  \\
No & 1036 (74.1\%) & 1887 (94.6\%) & 663 (70.2\%) & 591 (68.3\%) & 143 (33.2\%) & 260 (81.5\%) & 287 (96.0\%) & 89 (53.9\%) & 14 (18.4\%) & 28 (44.4\%) & 12 (21.1\%) & 12 (21.4\%) \\
Yes & 362 (25.9\%) & 107 (5.37\%) & 282 (29.8\%) & 274 (31.7\%) & 288 (66.8\%) & 59 (18.5\%) & 12 (4.01\%) & 76 (46.1\%) & 62 (81.6\%) & 35 (55.6\%) & 45 (78.9\%) & 44 (78.6\%) \\
Center A & Beijing Tsinghua Changgung Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center B & Tianjin Medical University Cancer Institute and Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center C & Zhongnan Hospital of Wuhan University &  &  &  &  &  &  &  &  &  &  &  \\
Center D & Mengchao Hepatobiliary Hospital of Fujian Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center E & Xingtai People's Hospital of Hebei Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center F & The Second Affiliated Hospital, Zhejiang University School of Medicine &  &  &  &  &  &  &  &  &  &  &  \\
Center G & Shenzhen People's Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center H & Southwest Hospital, Third Military Medical University (Army Medical University) &  &  &  &  &  &  &  &  &  &  &  \\
Center I & the Second Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center J & Guangxi Medical University First Affiliated Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center K & the Fourth Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center L & Peking Union Medical College Hospital &  &  &  &  &  &  &  &  &  &  &  \\
    \end{longtable}
    \end{center}
    \end{landscape}


==> table1_external_full.tex <==
% \begin{landscape}
% \begin{center}
% \scriptsize
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{longtable}{p{5.2cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}}
% \caption{Baseline characteristics of patients in the external multi-center HCC cohort (full dataset)}\label{tab:baseline_full_external}\\
% \toprule
% Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
% \midrule
% \endfirsthead
% \toprule
% \multicolumn{13}{l}{\small\emph{(continued)}}\\
% Characteristics & Center A & Center B & Center C & Center D & Center E & Center F & Center G & Center H & Center I & Center J & Center K & Center L \\
% \midrule
% \endhead
% \midrule
% \multicolumn{13}{r}{\small Continued on next page}\\
% \endfoot
% \bottomrule
% \endlastfoot
%  &      (N=1398)      &      (N=1994)      &      (N=945)       &      (N=865)       &      (N=431)       &      (N=319)       &      (N=299)       &      (N=165)       &       (N=76)       &       (N=63)       &       (N=57)       &       (N=56)       \\
% Sex, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     female &   260 (18.6\%)    &   406 (20.4\%)    &   213 (22.5\%)    &   109 (12.6\%)    &    93 (21.6\%)    &    55 (17.2\%)    &    47 (15.7\%)    &    29 (17.6\%)    &    10 (13.2\%)    &    9 (14.3\%)     &    9 (15.8\%)     &    8 (14.3\%)     \\
%     male &   1138 (81.4\%)   &   1588 (79.6\%)   &   732 (77.5\%)    &   756 (87.4\%)    &   338 (78.4\%)    &   264 (82.8\%)    &   252 (84.3\%)    &   136 (82.4\%)    &    66 (86.8\%)    &    54 (85.7\%)    &    48 (84.2\%)    &    48 (85.7\%)    \\
% Age (years), (median [IQR]) & 59.0 [51.0;66.0] & 60.0 [53.0;66.0] & 59.0 [50.0;66.0] & 57.0 [48.0;64.0] & 61.0 [53.0;67.0] & 61.0 [53.0;68.0] & 56.0 [47.0;65.0] & 52.0 [46.0;60.0] & 61.0 [51.0;69.0] & 54.0 [45.0;62.0] & 60.0 [52.0;65.0] & 54.5 [45.8;65.2] \\
% BMI (kg/m2), (median [IQR]) & 23.8 [21.5;25.8] & 24.2 [22.3;26.8] & 22.8 [20.8;24.8] & 23.7 [21.7;26.3] & 23.6 [21.4;26.0] & 23.5 [20.4;26.7] & 23.5 [21.3;25.6] & 23.4 [21.3;25.6] & 23.9 [22.4;26.1] & 23.5 [20.8;25.4] & 23.7 [21.2;26.8] & 24.3 [20.4;26.0] \\
% Diabetes, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   727 (73.7\%)    &   1603 (80.4\%)   &   696 (85.1\%)    &   682 (82.8\%)    &   286 (88.5\%)    &   254 (79.6\%)    &   252 (84.3\%)    &   136 (82.4\%)    &    57 (75.0\%)    &    56 (88.9\%)    &    40 (70.2\%)    &    51 (91.1\%)    \\
%     Yes &   260 (26.3\%)    &   391 (19.6\%)    &   122 (14.9\%)    &   142 (17.2\%)    &    37 (11.5\%)    &    65 (20.4\%)    &    47 (15.7\%)    &    29 (17.6\%)    &    19 (25.0\%)    &    7 (11.1\%)     &    17 (29.8\%)    &    5 (8.93\%)     \\
% Hypertension, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   660 (66.9\%)    &   1302 (65.3\%)   &   586 (77.4\%)    &   663 (80.5\%)    &   294 (74.8\%)    &   205 (64.3\%)    &   237 (79.3\%)    &   138 (83.6\%)    &    53 (69.7\%)    &    53 (84.1\%)    &    42 (73.7\%)    &    43 (76.8\%)    \\
%     Yes &   326 (33.1\%)    &   692 (34.7\%)    &   171 (22.6\%)    &   161 (19.5\%)    &    99 (25.2\%)    &   114 (35.7\%)    &    62 (20.7\%)    &    27 (16.4\%)    &    23 (30.3\%)    &    10 (15.9\%)    &    15 (26.3\%)    &    13 (23.2\%)    \\
% Cirrhosis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   412 (40.9\%)    &   444 (22.3\%)    &   363 (46.4\%)    &   429 (56.1\%)    &    39 (9.90\%)    &   138 (43.3\%)    &   122 (40.8\%)    &    59 (35.8\%)    &    9 (11.8\%)     &    18 (28.6\%)    &    15 (26.3\%)    &    7 (12.5\%)     \\
%     Yes &   596 (59.1\%)    &   1543 (77.7\%)   &   420 (53.6\%)    &   336 (43.9\%)    &   355 (90.1\%)    &   181 (56.7\%)    &   177 (59.2\%)    &   106 (64.2\%)    &    67 (88.2\%)    &    45 (71.4\%)    &    42 (73.7\%)    &    49 (87.5\%)    \\
% Chronic liver disease, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   182 (15.9\%)    &   192 (9.63\%)    &    47 (6.83\%)    &   124 (15.0\%)    &    30 (7.46\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.59\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     HBV &   850 (74.4\%)    &   1471 (73.8\%)   &   476 (69.2\%)    &   626 (76.0\%)    &   353 (87.8\%)    &   237 (74.3\%)    &   250 (83.6\%)    &   144 (87.3\%)    &    65 (85.5\%)    &    56 (88.9\%)    &    49 (86.0\%)    &    47 (83.9\%)    \\
%     HBV+HCV &    6 (0.53\%)     &    12 (0.60\%)    &    0 (0.00\%)     &    8 (0.97\%)     &    0 (0.00\%)     &    2 (0.63\%)     &    1 (0.33\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     HCV &    24 (2.10\%)    &   140 (7.02\%)    &    15 (2.18\%)    &    22 (2.67\%)    &    7 (1.74\%)     &    0 (0.00\%)     &    8 (2.68\%)     &    2 (1.21\%)     &    4 (5.26\%)     &    1 (1.59\%)     &    6 (10.5\%)     &    2 (3.57\%)     \\
%     Others &    80 (7.01\%)    &   179 (8.98\%)    &   150 (21.8\%)    &    44 (5.34\%)    &    12 (2.99\%)    &    80 (25.1\%)    &    40 (13.4\%)    &    19 (11.5\%)    &    7 (9.21\%)     &    5 (7.94\%)     &    2 (3.51\%)     &    7 (12.5\%)     \\
% ECOG PS, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     0 &   669 (54.9\%)    &   1228 (61.6\%)   &   248 (34.4\%)    &   467 (55.5\%)    &   144 (61.3\%)    &    319 (100\%)    &    66 (23.5\%)    &    67 (40.6\%)    &    38 (50.0\%)    &    21 (33.9\%)    &    30 (52.6\%)    &    27 (48.2\%)    \\
%     1 &   433 (35.6\%)    &   766 (38.4\%)    &   353 (49.0\%)    &   328 (39.0\%)    &    70 (29.8\%)    &    0 (0.00\%)     &   197 (70.1\%)    &    97 (58.8\%)    &    38 (50.0\%)    &    35 (56.5\%)    &    19 (33.3\%)    &    24 (42.9\%)    \\
%     2 &   110 (9.03\%)    &    0 (0.00\%)     &   113 (15.7\%)    &    47 (5.58\%)    &    21 (8.94\%)    &    0 (0.00\%)     &    18 (6.41\%)    &    1 (0.61\%)     &    0 (0.00\%)     &    5 (8.06\%)     &    8 (14.0\%)     &    5 (8.93\%)     \\
%     3 &    6 (0.49\%)     &    0 (0.00\%)     &    5 (0.69\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.61\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     4 &    0 (0.00\%)     &    0 (0.00\%)     &    1 (0.14\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% Child-Pugh stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     A &   810 (69.4\%)    &   1752 (88.0\%)   &   703 (85.1\%)    &   627 (74.5\%)    &   314 (79.7\%)    &   303 (95.0\%)    &   293 (98.0\%)    &   164 (99.4\%)    &    59 (77.6\%)    &    59 (93.7\%)    &    47 (82.5\%)    &    49 (87.5\%)    \\
%     B &   307 (26.3\%)    &   239 (12.0\%)    &   117 (14.2\%)    &   215 (25.5\%)    &    78 (19.8\%)    &    13 (4.08\%)    &    6 (2.01\%)     &    1 (0.61\%)     &    17 (22.4\%)    &    4 (6.35\%)     &    10 (17.5\%)    &    7 (12.5\%)     \\
%     C &    50 (4.28\%)    &    0 (0.00\%)     &    6 (0.73\%)     &    0 (0.00\%)     &    2 (0.51\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% mALBI\_stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     Grade 1 &   363 (33.2\%)    &   1498 (76.0\%)   &   331 (38.3\%)    &   289 (39.5\%)    &   145 (34.4\%)    &   210 (65.8\%)    &   225 (75.3\%)    &   126 (76.4\%)    &    26 (34.2\%)    &    36 (57.1\%)    &    32 (56.1\%)    &    26 (46.4\%)    \\
%     Grade 2a &   274 (25.0\%)    &   292 (14.8\%)    &   204 (23.6\%)    &   202 (27.6\%)    &    96 (22.8\%)    &    72 (22.6\%)    &    50 (16.7\%)    &    27 (16.4\%)    &    15 (19.7\%)    &    16 (25.4\%)    &    6 (10.5\%)     &    10 (17.9\%)    \\
%     Grade 2b &   392 (35.8\%)    &   172 (8.73\%)    &   238 (27.5\%)    &   220 (30.1\%)    &   171 (40.6\%)    &    35 (11.0\%)    &    23 (7.69\%)    &    11 (6.67\%)    &    29 (38.2\%)    &    10 (15.9\%)    &    17 (29.8\%)    &    19 (33.9\%)    \\
%     Grade 3 &    66 (6.03\%)    &    8 (0.41\%)     &    92 (10.6\%)    &    21 (2.87\%)    &    9 (2.14\%)     &    2 (0.63\%)     &    1 (0.33\%)     &    1 (0.61\%)     &    6 (7.89\%)     &    1 (1.59\%)     &    2 (3.51\%)     &    1 (1.79\%)     \\
% WBC (109/L), (median [IQR]) & 4.69 [3.47;6.26] & 5.11 [4.08;6.29] & 5.38 [4.20;7.40] & 5.50 [4.10;7.17] & 5.00 [3.80;6.30] & 5.60 [4.50;7.00] & 5.56 [4.50;7.04] & 5.18 [4.29;6.57] & 4.80 [3.88;6.15] & 6.26 [5.30;7.62] & 5.20 [3.40;6.40] & 4.55 [3.10;5.85] \\
% NEUT (109/L), (median [IQR]) & 3.06 [2.12;4.50] & 2.86 [2.15;3.74] & 3.50 [2.40;5.68] & 3.40 [2.40;4.80] & 2.90 [2.16;4.10] & 3.57 [2.66;4.64] & 3.00 [2.40;4.15] & 3.24 [2.51;4.08] & 3.15 [2.40;4.60] & 3.89 [3.12;5.14] & 3.70 [2.50;4.70] & 3.25 [2.28;4.50] \\
% LYMPH (109/L), (median [IQR]) & 1.01 [0.61;1.46] & 1.54 [1.19;1.96] & 1.17 [0.80;1.50] & 1.28 [0.88;1.74] & 1.30 [0.90;1.70] & 1.48 [1.07;1.85] & 1.68 [1.31;2.09] & 1.35 [1.02;1.71] & 0.90 [0.70;1.40] & 1.67 [1.30;2.03] & 1.10 [0.70;1.50] & 0.85 [0.60;1.20] \\
% RBC (1012/L), (median [IQR]) & 4.03 [3.48;4.51] & 4.62 [4.23;4.98] & 4.09 [3.66;4.56] & 4.48 [3.92;5.00] & 4.06 [3.59;4.45] & 4.52 [4.12;4.88] & 4.70 [4.34;5.18] & 4.76 [4.40;5.11] & 4.40 [3.58;5.00] & 4.59 [4.25;4.86] & 4.40 [3.60;5.00] & 4.25 [3.18;4.82] \\
% HGB (g/L), (median [IQR]) &  126 [110;139]   &  145 [133;155]   &  131 [116;142]   &  138 [123;152]   &  130 [118;143]   &  142 [128;154]   &  144 [128;154]   &  146 [133;156]   &  137 [120;152]   &  139 [126;145]   &  135 [120;150]   &  132 [115;147]   \\
% PLT (109/L), (median [IQR]) &  135 [86.2;191]  &  153 [110;200]   &  154 [113;205]   &  158 [111;222]   &  124 [79.8;177]  &  156 [118;196]   &  184 [132;227]   &  160 [123;216]   &  159 [98.5;206]  &  220 [158;282]   &  152 [104;227]   &  148 [98.2;210]  \\
% ALT (U/L), (median [IQR]) & 27.7 [17.6;47.4] & 25.0 [17.0;38.0] & 28.0 [18.0;47.0] & 35.0 [22.9;53.0] & 30.8 [21.0;45.7] & 30.0 [21.0;44.0] & 29.0 [22.0;41.0] & 30.1 [22.2;43.9] & 37.4 [24.0;51.4] & 31.0 [25.5;50.5] & 30.0 [15.8;43.1] & 32.2 [19.5;47.2] \\
% AST (U/L), (median [IQR]) & 39.3 [25.0;78.3] & 26.0 [20.0;37.0] & 31.0 [22.0;46.0] & 42.0 [29.4;68.9] & 35.6 [25.0;54.8] & 34.0 [25.5;49.0] & 28.0 [22.0;40.0] & 31.9 [26.2;41.8] & 47.0 [31.5;70.7] & 42.0 [26.0;60.5] & 37.2 [27.4;67.0] & 44.9 [30.6;69.2] \\
% TBIL (\$\mu\$mmol/L), (median [IQR]) & 15.3 [10.3;27.6] & 14.0 [10.3;18.7] & 15.6 [11.6;21.2] & 17.5 [12.7;24.1] & 18.1 [13.5;25.5] & 15.3 [11.7;20.4] & 13.3 [9.75;16.9] & 15.1 [12.1;19.6] & 18.9 [15.0;31.5] & 12.4 [8.15;18.8] & 16.2 [11.2;22.0] & 17.9 [10.9;28.1] \\
% DBIL (umol/L), (median [IQR]) & 6.80 [4.60;14.2] & 5.50 [4.20;7.60] & 3.90 [2.70;6.10] & 6.70 [4.60;10.0] & 6.50 [4.40;10.1] & 3.10 [2.30;4.45] & 4.59 [3.50;6.06] & 2.83 [2.20;3.70] & 8.25 [5.65;17.5] & 4.10 [3.15;6.55] & 7.30 [4.40;12.4] & 6.90 [4.88;12.1] \\
% ALB (g/L), (median [IQR]) & 37.1 [33.9;40.3] & 42.5 [39.7;45.4] & 38.3 [34.9;41.9] & 38.2 [35.3;42.0] & 37.7 [34.2;41.6] & 41.1 [38.7;43.5] & 42.2 [39.3;44.8] & 42.8 [39.8;45.8] & 37.8 [34.6;40.9] & 38.9 [36.0;41.9] & 40.6 [35.5;44.1] & 38.8 [35.0;43.2] \\
% GGT (U/L), (median [IQR]) & 72.0 [37.0;162]  & 44.0 [27.0;79.0] & 58.5 [31.0;121]  & 96.0 [48.0;180]  & 59.0 [32.0;117]  & 53.0 [27.5;105]  & 41.0 [27.0;80.0] & 48.3 [29.0;95.5] &  107 [56.6;211]  &  106 [55.0;196]  & 97.5 [39.7;198]  & 95.7 [50.0;190]  \\
% ALP (U/L), (median [IQR]) &  102 [76.0;152]  & 85.0 [69.0;108]  & 97.0 [76.0;132]  &  110 [84.5;160]  &  106 [78.0;146]  & 96.5 [78.0;128]  & 74.0 [61.0;94.0] & 93.1 [77.7;111]  &  135 [93.3;229]  &  110 [80.0;152]  &  114 [92.0;181]  &  118 [80.9;199]  \\
% Cre (\$\mu\$mol/L), (median [IQR]) & 67.0 [57.0;78.0] & 69.0 [60.0;78.0] & 67.9 [59.3;78.7] & 67.0 [58.0;76.0] & 63.5 [55.1;73.7] & 71.4 [62.2;80.2] & 81.0 [68.0;93.0] & 75.8 [68.1;83.8] & 59.3 [51.8;71.6] & 73.0 [66.0;78.0] & 60.3 [51.4;69.0] & 65.4 [54.9;74.5] \\
% BUN (mmol/L), (median [IQR]) & 5.00 [3.90;6.30] & 5.20 [4.30;6.20] & 5.21 [4.20;6.36] & 4.50 [3.60;5.70] & 4.75 [3.98;5.83] & 5.38 [4.38;6.43] & 4.90 [4.11;5.68] & 5.48 [4.50;6.33] & 4.90 [3.58;5.82] & 4.49 [3.37;5.46] & 5.10 [3.80;6.00] & 4.80 [4.05;5.90] \\
% UA (\$\mu\$mol/L), (median [IQR]) &  308 [253;386]   &  306 [256;361]   &  301 [235;367]   &  311 [253;376]   &  271 [213;333]   &  323 [276;377]   &  315 [284;360]   &  346 [285;406]   &  298 [219;336]   &  320 [268;370]   &  299 [251;336]   &  287 [231;352]   \\
% GLU (mmol/L), (median [IQR]) & 5.46 [4.87;7.26] & 5.25 [4.77;6.15] & 5.11 [4.58;6.18] & 5.38 [4.78;6.22] & 5.38 [4.84;6.20] & 5.58 [4.99;6.49] & 5.08 [4.89;5.72] & 5.28 [4.77;6.10] & 5.45 [4.90;6.50] & 5.80 [5.00;7.28] & 5.50 [5.00;6.40] & 5.60 [4.90;6.50] \\
% PT (s), (median [IQR]) & 12.6 [11.9;14.2] & 11.9 [11.3;12.5] & 12.2 [11.4;13.0] & 13.1 [12.3;14.0] & 12.1 [11.3;12.9] & 13.2 [12.8;13.8] & 12.3 [11.7;13.0] & 11.7 [11.3;12.2] & 13.0 [12.0;13.9] & 11.9 [11.3;12.6] & 12.6 [11.8;13.9] & 12.9 [12.1;13.6] \\
% INR, (median [IQR]) & 1.08 [1.02;1.23] & 1.03 [0.98;1.09] & 1.12 [1.04;1.19] & 1.04 [1.00;1.10] & 1.10 [1.04;1.19] & 1.02 [0.97;1.07] & 1.01 [0.96;1.06] & 1.04 [1.00;1.08] & 1.10 [1.00;1.20] & 1.05 [1.00;1.12] & 1.10 [1.00;1.20] & 1.10 [1.00;1.20] \\
% APTT (s), (median [IQR]) & 28.8 [27.1;31.9] & 26.8 [24.9;29.3] & 31.3 [29.3;33.7] & 33.9 [28.5;37.7] & 34.1 [31.5;37.1] & 35.0 [33.0;37.8] & 32.3 [29.9;34.6] & 27.6 [26.2;29.0] & 28.6 [27.0;31.0] & 32.7 [30.7;34.6] & 27.7 [26.6;31.1] & 28.9 [27.1;30.9] \\
% Fib (g/L), (median [IQR]) & 2.43 [1.82;3.18] & 2.55 [2.18;3.09] &  309 [248;393]   & 3.30 [2.68;4.11] & 2.66 [2.21;3.25] & 2.96 [2.42;3.57] & 2.81 [2.39;3.41] & 2.53 [2.20;2.97] & 3.55 [2.77;4.60] & 3.38 [2.81;4.07] & 3.50 [2.90;5.10] & 3.80 [2.90;4.95] \\
% AFP, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     <=400 &   827 (78.5\%)    &   1608 (82.9\%)   &   578 (77.4\%)    &   259 (43.1\%)    &   341 (85.0\%)    &   238 (75.1\%)    &   235 (78.6\%)    &   115 (71.0\%)    &    33 (43.4\%)    &    37 (58.7\%)    &    26 (45.6\%)    &    18 (32.1\%)    \\
%     >400 &   227 (21.5\%)    &   332 (17.1\%)    &   169 (22.6\%)    &   342 (56.9\%)    &    60 (15.0\%)    &    79 (24.9\%)    &    64 (21.4\%)    &    47 (29.0\%)    &    43 (56.6\%)    &    26 (41.3\%)    &    31 (54.4\%)    &    38 (67.9\%)    \\
% PIVKA-II, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     <=1000 &   759 (73.6\%)    &   844 (85.7\%)    &   171 (65.8\%)    &   258 (45.9\%)    &      0 (.\%)      &   135 (79.4\%)    &    16 (72.7\%)    &   121 (76.6\%)    &    40 (52.6\%)    &    34 (54.0\%)    &    30 (52.6\%)    &    28 (50.0\%)    \\
%     >1000 &   272 (26.4\%)    &   141 (14.3\%)    &    89 (34.2\%)    &   304 (54.1\%)    &      0 (.\%)      &    35 (20.6\%)    &    6 (27.3\%)     &    37 (23.4\%)    &    36 (47.4\%)    &    29 (46.0\%)    &    27 (47.4\%)    &    28 (50.0\%)    \\
% Tumor numbers, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     1 &   675 (57.9\%)    &   1491 (75.3\%)   &   529 (75.5\%)    &   431 (52.5\%)    &   225 (66.8\%)    &   268 (84.3\%)    &   284 (95.0\%)    &   147 (89.1\%)    &    3 (3.95\%)     &    34 (54.8\%)    &    2 (3.51\%)     &    7 (12.5\%)     \\
%     2 &   160 (13.7\%)    &   315 (15.9\%)    &   105 (15.0\%)    &    93 (11.3\%)    &    36 (10.7\%)    &    25 (7.86\%)    &    12 (4.01\%)    &    7 (4.24\%)     &    13 (17.1\%)    &    12 (19.4\%)    &    3 (5.26\%)     &    7 (12.5\%)     \\
%     3 &    85 (7.29\%)    &    67 (3.38\%)    &    19 (2.71\%)    &    55 (6.70\%)    &    6 (1.78\%)     &    5 (1.57\%)     &    3 (1.00\%)     &    1 (0.61\%)     &    5 (6.58\%)     &    1 (1.61\%)     &    9 (15.8\%)     &    3 (5.36\%)     \\
%     >=4 &   246 (21.1\%)    &   107 (5.40\%)    &    48 (6.85\%)    &   242 (29.5\%)    &    70 (20.8\%)    &    20 (6.29\%)    &    0 (0.00\%)     &    10 (6.06\%)    &    55 (72.4\%)    &    15 (24.2\%)    &    43 (75.4\%)    &    39 (69.6\%)    \\
% Tumor maximum diameter, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     <=3 &   341 (29.8\%)    &   1023 (51.7\%)   &   161 (23.9\%)    &   150 (17.4\%)    &    90 (28.2\%)    &   120 (37.7\%)    &    97 (38.6\%)    &    48 (29.1\%)    &    3 (3.95\%)     &    12 (19.4\%)    &    3 (5.26\%)     &    6 (10.7\%)     \\
%     >3, <=5 &   274 (23.9\%)    &   539 (27.3\%)    &   174 (25.8\%)    &   109 (12.6\%)    &    78 (24.5\%)    &    91 (28.6\%)    &    67 (26.7\%)    &    46 (27.9\%)    &    3 (3.95\%)     &    11 (17.7\%)    &    6 (10.5\%)     &    0 (0.00\%)     \\
%     >5 &   531 (46.3\%)    &   415 (21.0\%)    &   340 (50.4\%)    &   605 (70.0\%)    &   151 (47.3\%)    &   107 (33.6\%)    &    87 (34.7\%)    &    71 (43.0\%)    &    70 (92.1\%)    &    39 (62.9\%)    &    48 (84.2\%)    &    50 (89.3\%)    \\
% Vessel invasion, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   898 (75.7\%)    &   1901 (96.0\%)   &   453 (64.3\%)    &   471 (54.5\%)    &   182 (76.8\%)    &   301 (94.4\%)    &   291 (97.3\%)    &   125 (75.8\%)    &    24 (31.6\%)    &    50 (79.4\%)    &    18 (31.6\%)    &    16 (28.6\%)    \\
%     Yes &   288 (24.3\%)    &    79 (3.99\%)    &   252 (35.7\%)    &   394 (45.5\%)    &    55 (23.2\%)    &    18 (5.64\%)    &    8 (2.68\%)     &    40 (24.2\%)    &    52 (68.4\%)    &    13 (20.6\%)    &    39 (68.4\%)    &    40 (71.4\%)    \\
% Lymph Node Metastasis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   879 (87.8\%)    &   1738 (87.8\%)   &   603 (85.9\%)    &   800 (92.5\%)    &   378 (87.7\%)    &   314 (98.4\%)    &   295 (98.7\%)    &    165 (100\%)    &    70 (92.1\%)    &    55 (87.3\%)    &    48 (84.2\%)    &    49 (87.5\%)    \\
%     Yes &   122 (12.2\%)    &   241 (12.2\%)    &    99 (14.1\%)    &    65 (7.51\%)    &    53 (12.3\%)    &    5 (1.57\%)     &    4 (1.34\%)     &    0 (0.00\%)     &    6 (7.89\%)     &    8 (12.7\%)     &    9 (15.8\%)     &    7 (12.5\%)     \\
% Distant Metastasis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   870 (86.1\%)    &   1926 (97.3\%)   &   636 (90.3\%)    &   757 (87.5\%)    &   376 (87.2\%)    &   317 (99.4\%)    &    299 (100\%)    &   162 (99.4\%)    &    62 (81.6\%)    &    52 (82.5\%)    &    35 (61.4\%)    &    45 (80.4\%)    \\
%     Yes &   140 (13.9\%)    &    53 (2.68\%)    &    68 (9.66\%)    &   108 (12.5\%)    &    55 (12.8\%)    &    2 (0.63\%)     &    0 (0.00\%)     &    1 (0.61\%)     &    14 (18.4\%)    &    11 (17.5\%)    &    22 (38.6\%)    &    11 (19.6\%)    \\
% BCLC stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     0 &    98 (9.91\%)    &   354 (17.9\%)    &    36 (5.68\%)    &    32 (3.80\%)    &    13 (5.51\%)    &    59 (18.5\%)    &    37 (14.7\%)    &    19 (11.7\%)    &    0 (0.00\%)     &    6 (9.68\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     A &   382 (38.6\%)    &   1068 (54.1\%)   &   249 (39.3\%)    &   264 (31.4\%)    &    92 (39.0\%)    &   199 (62.4\%)    &   195 (77.7\%)    &    95 (58.3\%)    &    0 (0.00\%)     &    20 (32.3\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
%     B &   131 (13.2\%)    &   223 (11.3\%)    &    58 (9.15\%)    &   123 (14.6\%)    &    32 (13.6\%)    &    35 (11.0\%)    &    8 (3.19\%)     &    9 (5.52\%)     &    23 (30.3\%)    &    17 (27.4\%)    &    16 (28.1\%)    &    15 (26.8\%)    \\
%     C &   328 (33.2\%)    &   329 (16.7\%)    &   285 (45.0\%)    &   423 (50.2\%)    &    97 (41.1\%)    &    23 (7.21\%)    &    11 (4.38\%)    &    40 (24.5\%)    &    53 (69.7\%)    &    19 (30.6\%)    &    41 (71.9\%)    &    41 (73.2\%)    \\
%     D &    50 (5.06\%)    &    0 (0.00\%)     &    6 (0.95\%)     &    0 (0.00\%)     &    2 (0.85\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% CNLC stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     Ia &   300 (30.2\%)    &   1050 (53.2\%)   &   155 (24.3\%)    &   131 (15.6\%)    &    64 (27.1\%)    &   181 (56.7\%)    &   149 (59.4\%)    &    65 (39.9\%)    &    0 (0.00\%)     &    15 (24.2\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
%     Ib &   179 (18.0\%)    &   372 (18.8\%)    &   128 (20.1\%)    &   165 (19.6\%)    &    41 (17.4\%)    &    77 (24.1\%)    &    83 (33.1\%)    &    49 (30.1\%)    &    0 (0.00\%)     &    11 (17.7\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
%     IIa &    80 (8.06\%)    &   164 (8.31\%)    &    41 (6.44\%)    &    55 (6.53\%)    &    14 (5.93\%)    &    20 (6.27\%)    &    8 (3.19\%)     &    2 (1.23\%)     &    0 (0.00\%)     &    10 (16.1\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
%     IIb &    51 (5.14\%)    &    59 (2.99\%)    &    16 (2.51\%)    &    68 (8.08\%)    &    18 (7.63\%)    &    15 (4.70\%)    &    0 (0.00\%)     &    7 (4.29\%)     &    23 (30.3\%)    &    7 (11.3\%)     &    16 (28.1\%)    &    15 (26.8\%)    \\
%     IIIa &   152 (15.3\%)    &    50 (2.53\%)    &   178 (27.9\%)    &   282 (33.5\%)    &    34 (14.4\%)    &    16 (5.02\%)    &    7 (2.79\%)     &    39 (23.9\%)    &    36 (47.4\%)    &    6 (9.68\%)     &    16 (28.1\%)    &    28 (50.0\%)    \\
%     IIIb &   175 (17.6\%)    &   279 (14.1\%)    &   107 (16.8\%)    &   141 (16.7\%)    &    63 (26.7\%)    &    7 (2.19\%)     &    4 (1.59\%)     &    1 (0.61\%)     &    17 (22.4\%)    &    12 (19.4\%)    &    25 (43.9\%)    &    13 (23.2\%)    \\
%     IV &    56 (5.64\%)    &    0 (0.00\%)     &    12 (1.88\%)    &    0 (0.00\%)     &    2 (0.85\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.61\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% TNM stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     IA &   105 (10.7\%)    &   354 (17.9\%)    &    36 (5.76\%)    &    32 (3.81\%)    &    13 (5.78\%)    &    60 (18.8\%)    &    37 (14.7\%)    &    19 (11.7\%)    &    0 (0.00\%)     &    6 (9.84\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     IB &   339 (34.6\%)    &   917 (46.5\%)    &   241 (38.6\%)    &   244 (29.0\%)    &    86 (38.2\%)    &   193 (60.5\%)    &   190 (75.7\%)    &    92 (56.4\%)    &    0 (0.00\%)     &    19 (31.1\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
%     II &   138 (14.1\%)    &   285 (14.4\%)    &    38 (6.08\%)    &    59 (7.02\%)    &    20 (8.89\%)    &    25 (7.84\%)    &    11 (4.38\%)    &    12 (7.36\%)    &    2 (2.63\%)     &    7 (11.5\%)     &    1 (1.75\%)     &    4 (7.14\%)     \\
%     IIIA &    64 (6.54\%)    &    89 (4.51\%)    &    30 (4.80\%)    &    84 (10.0\%)    &    16 (7.11\%)    &    18 (5.64\%)    &    2 (0.80\%)     &    0 (0.00\%)     &    21 (27.6\%)    &    11 (18.0\%)    &    15 (26.3\%)    &    11 (19.6\%)    \\
%     IIIB &   166 (17.0\%)    &    50 (2.53\%)    &   178 (28.5\%)    &   282 (33.6\%)    &    34 (15.1\%)    &    16 (5.02\%)    &    7 (2.79\%)     &    39 (23.9\%)    &    36 (47.4\%)    &    6 (9.84\%)     &    16 (28.1\%)    &    28 (50.0\%)    \\
%     IVA &    51 (5.21\%)    &   227 (11.5\%)    &    45 (7.20\%)    &    31 (3.69\%)    &    29 (12.9\%)    &    5 (1.57\%)     &    4 (1.59\%)     &    0 (0.00\%)     &    3 (3.95\%)     &    1 (1.64\%)     &    3 (5.26\%)     &    2 (3.57\%)     \\
%     IVB &   116 (11.8\%)    &    52 (2.63\%)    &    57 (9.12\%)    &   108 (12.9\%)    &    27 (12.0\%)    &    2 (0.63\%)     &    0 (0.00\%)     &    1 (0.61\%)     &    14 (18.4\%)    &    11 (18.0\%)    &    22 (38.6\%)    &    11 (19.6\%)    \\
% Surgery, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   635 (45.4\%)    &   866 (43.4\%)    &   309 (32.7\%)    &   323 (37.3\%)    &   323 (74.9\%)    &    30 (9.40\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    76 (100\%)     &    41 (65.1\%)    &    57 (100\%)     &    56 (100\%)     \\
%     Yes &   763 (54.6\%)    &   1128 (56.6\%)   &   636 (67.3\%)    &   542 (62.7\%)    &   108 (25.1\%)    &   289 (90.6\%)    &    299 (100\%)    &    165 (100\%)    &    0 (0.00\%)     &    22 (34.9\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
% RFA, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   1290 (92.3\%)   &   1209 (60.6\%)   &   902 (95.4\%)    &    865 (100\%)    &    431 (100\%)    &   303 (95.0\%)    &    299 (100\%)    &   116 (70.3\%)    &    76 (100\%)     &    58 (92.1\%)    &    57 (100\%)     &    56 (100\%)     \\
%     Yes &   108 (7.73\%)    &   785 (39.4\%)    &    43 (4.55\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    16 (5.02\%)    &    0 (0.00\%)     &    49 (29.7\%)    &    0 (0.00\%)     &    5 (7.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% TACE, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   892 (63.8\%)    &   1914 (96.0\%)   &   863 (91.3\%)    &   679 (78.5\%)    &   108 (25.1\%)    &   302 (94.7\%)    &    299 (100\%)    &   159 (96.4\%)    &    30 (39.5\%)    &    34 (54.0\%)    &    22 (38.6\%)    &    22 (39.3\%)    \\
%     Yes &   506 (36.2\%)    &    80 (4.01\%)    &    82 (8.68\%)    &   186 (21.5\%)    &   323 (74.9\%)    &    17 (5.33\%)    &    0 (0.00\%)     &    6 (3.64\%)     &    46 (60.5\%)    &    29 (46.0\%)    &    35 (61.4\%)    &    34 (60.7\%)    \\
% HAIC, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   1181 (84.5\%)   &   1943 (97.4\%)   &   938 (99.3\%)    &   840 (97.1\%)    &    431 (100\%)    &   318 (99.7\%)    &    299 (100\%)    &   162 (98.2\%)    &    76 (100\%)     &    38 (60.3\%)    &    57 (100\%)     &    42 (75.0\%)    \\
%     Yes &   217 (15.5\%)    &    51 (2.56\%)    &    7 (0.74\%)     &    25 (2.89\%)    &    0 (0.00\%)     &    1 (0.31\%)     &    0 (0.00\%)     &    3 (1.82\%)     &    0 (0.00\%)     &    25 (39.7\%)    &    0 (0.00\%)     &    14 (25.0\%)    \\
% EBRT, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   1319 (94.3\%)   &   1994 (100\%)    &    945 (100\%)    &   542 (62.7\%)    &    431 (100\%)    &    319 (100\%)    &    299 (100\%)    &    165 (100\%)    &    0 (0.00\%)     &    63 (100\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
%     Yes &    79 (5.65\%)    &    0 (0.00\%)     &    0 (0.00\%)     &   323 (37.3\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    76 (100\%)     &    0 (0.00\%)     &    57 (100\%)     &    56 (100\%)     \\
% SIRT, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   976 (69.8\%)    &   1994 (100\%)    &    945 (100\%)    &    865 (100\%)    &    431 (100\%)    &    319 (100\%)    &    299 (100\%)    &    165 (100\%)    &    76 (100\%)     &    63 (100\%)     &    57 (100\%)     &    56 (100\%)     \\
%     Yes &   422 (30.2\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
% TKI, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   972 (69.5\%)    &   1898 (95.2\%)   &   639 (67.6\%)    &   578 (66.8\%)    &   137 (31.8\%)    &   296 (92.8\%)    &   287 (96.0\%)    &    99 (60.0\%)    &    10 (13.2\%)    &    24 (38.1\%)    &    8 (14.0\%)     &    6 (10.7\%)     \\
%     Yes &   426 (30.5\%)    &    96 (4.81\%)    &   306 (32.4\%)    &   287 (33.2\%)    &   294 (68.2\%)    &    23 (7.21\%)    &    12 (4.01\%)    &    66 (40.0\%)    &    66 (86.8\%)    &    39 (61.9\%)    &    49 (86.0\%)    &    50 (89.3\%)    \\
% ICIs, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
%     No &   1036 (74.1\%)   &   1887 (94.6\%)   &   663 (70.2\%)    &   591 (68.3\%)    &   143 (33.2\%)    &   260 (81.5\%)    &   287 (96.0\%)    &    89 (53.9\%)    &    14 (18.4\%)    &    28 (44.4\%)    &    12 (21.1\%)    &    12 (21.4\%)    \\
%     Yes &   362 (25.9\%)    &   107 (5.37\%)    &   282 (29.8\%)    &   274 (31.7\%)    &   288 (66.8\%)    &    59 (18.5\%)    &    12 (4.01\%)    &    76 (46.1\%)    &    62 (81.6\%)    &    35 (55.6\%)    &    45 (78.9\%)    &    44 (78.6\%)    \\
%  &  &  &  &  &  &  &  &  &  &  &  &  \\
% Center A & Beijing Tsinghua Changgung Hospital &  &  &  &  &  &  &  &  &  &  &  \\
% Center B & Tianjin Medical University Cancer Institute and Hospital &  &  &  &  &  &  &  &  &  &  &  \\
% Center C & Zhongnan Hospital of Wuhan University &  &  &  &  &  &  &  &  &  &  &  \\
% Center D & Mengchao Hepatobiliary Hospital of Fujian Medical University &  &  &  &  &  &  &  &  &  &  &  \\
% Center E & Xingtai People's Hospital of Hebei Medical University &  &  &  &  &  &  &  &  &  &  &  \\
% Center F & The Second Affiliated Hospital, Zhejiang University School of Medicine &  &  &  &  &  &  &  &  &  &  &  \\
% Center G & Shenzhen People's Hospital &  &  &  &  &  &  &  &  &  &  &  \\
% Center H & Southwest Hospital, Third Military Medical University (Army Medical University) &  &  &  &  &  &  &  &  &  &  &  \\
% Center I & the Second Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
% Center J & Guangxi Medical University First Affiliated Hospital &  &  &  &  &  &  &  &  &  &  &  \\
% Center K & the Fourth Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
% Center L & Peking Union Medical College Hospital &  &  &  &  &  &  &  &  &  &  &  \\
% \end{longtable}
% \end{center}
% \end{landscape}




\captionsetup[table]{skip=6pt}
\newcommand{\rot}[1]{\rotatebox[origin=c]{90}{\footnotesize #1}}

\begin{landscape}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{center}
\begin{longtable}{p{6.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}p{3.0cm}}
\caption{Baseline characteristics of patients in the external multi-center HCC cohort (full dataset)}\label{tab:baseline_full_external}\\
\toprule
\small Characteristics & \rot{Center A} & \rot{Center B} & \rot{Center C} & \rot{Center D} & \rot{Center E} & \rot{Center F} & \rot{Center G} & \rot{Center H} & \rot{Center I} & \rot{Center J} & \rot{Center K} & \rot{Center L} \\
\midrule
\endfirsthead
\toprule
\multicolumn{13}{l}{\small\emph{(continued)}}\\
\small Characteristics & \rot{Center A} & \rot{Center B} & \rot{Center C} & \rot{Center D} & \rot{Center E} & \rot{Center F} & \rot{Center G} & \rot{Center H} & \rot{Center I} & \rot{Center J} & \rot{Center K} & \rot{Center L} \\
\midrule
\endhead
\midrule
\multicolumn{13}{r}{\small Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
 &      (N=1398)      &      (N=1994)      &      (N=945)       &      (N=865)       &      (N=431)       &      (N=319)       &      (N=299)       &      (N=165)       &       (N=76)       &       (N=63)       &       (N=57)       &       (N=56)       \\
Sex, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    female &   260 (18.6\%)    &   406 (20.4\%)    &   213 (22.5\%)    &   109 (12.6\%)    &    93 (21.6\%)    &    55 (17.2\%)    &    47 (15.7\%)    &    29 (17.6\%)    &    10 (13.2\%)    &    9 (14.3\%)     &    9 (15.8\%)     &    8 (14.3\%)     \\
    male &   1138 (81.4\%)   &   1588 (79.6\%)   &   732 (77.5\%)    &   756 (87.4\%)    &   338 (78.4\%)    &   264 (82.8\%)    &   252 (84.3\%)    &   136 (82.4\%)    &    66 (86.8\%)    &    54 (85.7\%)    &    48 (84.2\%)    &    48 (85.7\%)    \\
Age (years), (median [IQR]) & 59.0 [51.0;66.0] & 60.0 [53.0;66.0] & 59.0 [50.0;66.0] & 57.0 [48.0;64.0] & 61.0 [53.0;67.0] & 61.0 [53.0;68.0] & 56.0 [47.0;65.0] & 52.0 [46.0;60.0] & 61.0 [51.0;69.0] & 54.0 [45.0;62.0] & 60.0 [52.0;65.0] & 54.5 [45.8;65.2] \\
BMI (kg/m2), (median [IQR]) & 23.8 [21.5;25.8] & 24.2 [22.3;26.8] & 22.8 [20.8;24.8] & 23.7 [21.7;26.3] & 23.6 [21.4;26.0] & 23.5 [20.4;26.7] & 23.5 [21.3;25.6] & 23.4 [21.3;25.6] & 23.9 [22.4;26.1] & 23.5 [20.8;25.4] & 23.7 [21.2;26.8] & 24.3 [20.4;26.0] \\
Diabetes, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   727 (73.7\%)    &   1603 (80.4\%)   &   696 (85.1\%)    &   682 (82.8\%)    &   286 (88.5\%)    &   254 (79.6\%)    &   252 (84.3\%)    &   136 (82.4\%)    &    57 (75.0\%)    &    56 (88.9\%)    &    40 (70.2\%)    &    51 (91.1\%)    \\
    Yes &   260 (26.3\%)    &   391 (19.6\%)    &   122 (14.9\%)    &   142 (17.2\%)    &    37 (11.5\%)    &    65 (20.4\%)    &    47 (15.7\%)    &    29 (17.6\%)    &    19 (25.0\%)    &    7 (11.1\%)     &    17 (29.8\%)    &    5 (8.93\%)     \\
Hypertension, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   660 (66.9\%)    &   1302 (65.3\%)   &   586 (77.4\%)    &   663 (80.5\%)    &   294 (74.8\%)    &   205 (64.3\%)    &   237 (79.3\%)    &   138 (83.6\%)    &    53 (69.7\%)    &    53 (84.1\%)    &    42 (73.7\%)    &    43 (76.8\%)    \\
    Yes &   326 (33.1\%)    &   692 (34.7\%)    &   171 (22.6\%)    &   161 (19.5\%)    &    99 (25.2\%)    &   114 (35.7\%)    &    62 (20.7\%)    &    27 (16.4\%)    &    23 (30.3\%)    &    10 (15.9\%)    &    15 (26.3\%)    &    13 (23.2\%)    \\
Cirrhosis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   412 (40.9\%)    &   444 (22.3\%)    &   363 (46.4\%)    &   429 (56.1\%)    &    39 (9.90\%)    &   138 (43.3\%)    &   122 (40.8\%)    &    59 (35.8\%)    &    9 (11.8\%)     &    18 (28.6\%)    &    15 (26.3\%)    &    7 (12.5\%)     \\
    Yes &   596 (59.1\%)    &   1543 (77.7\%)   &   420 (53.6\%)    &   336 (43.9\%)    &   355 (90.1\%)    &   181 (56.7\%)    &   177 (59.2\%)    &   106 (64.2\%)    &    67 (88.2\%)    &    45 (71.4\%)    &    42 (73.7\%)    &    49 (87.5\%)    \\
Chronic liver disease, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   182 (15.9\%)    &   192 (9.63\%)    &    47 (6.83\%)    &   124 (15.0\%)    &    30 (7.46\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.59\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    HBV &   850 (74.4\%)    &   1471 (73.8\%)   &   476 (69.2\%)    &   626 (76.0\%)    &   353 (87.8\%)    &   237 (74.3\%)    &   250 (83.6\%)    &   144 (87.3\%)    &    65 (85.5\%)    &    56 (88.9\%)    &    49 (86.0\%)    &    47 (83.9\%)    \\
    HBV+HCV &    6 (0.53\%)     &    12 (0.60\%)    &    0 (0.00\%)     &    8 (0.97\%)     &    0 (0.00\%)     &    2 (0.63\%)     &    1 (0.33\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    HCV &    24 (2.10\%)    &   140 (7.02\%)    &    15 (2.18\%)    &    22 (2.67\%)    &    7 (1.74\%)     &    0 (0.00\%)     &    8 (2.68\%)     &    2 (1.21\%)     &    4 (5.26\%)     &    1 (1.59\%)     &    6 (10.5\%)     &    2 (3.57\%)     \\
    Others &    80 (7.01\%)    &   179 (8.98\%)    &   150 (21.8\%)    &    44 (5.34\%)    &    12 (2.99\%)    &    80 (25.1\%)    &    40 (13.4\%)    &    19 (11.5\%)    &    7 (9.21\%)     &    5 (7.94\%)     &    2 (3.51\%)     &    7 (12.5\%)     \\
ECOG PS, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    0 &   669 (54.9\%)    &   1228 (61.6\%)   &   248 (34.4\%)    &   467 (55.5\%)    &   144 (61.3\%)    &    319 (100\%)    &    66 (23.5\%)    &    67 (40.6\%)    &    38 (50.0\%)    &    21 (33.9\%)    &    30 (52.6\%)    &    27 (48.2\%)    \\
    1 &   433 (35.6\%)    &   766 (38.4\%)    &   353 (49.0\%)    &   328 (39.0\%)    &    70 (29.8\%)    &    0 (0.00\%)     &   197 (70.1\%)    &    97 (58.8\%)    &    38 (50.0\%)    &    35 (56.5\%)    &    19 (33.3\%)    &    24 (42.9\%)    \\
    2 &   110 (9.03\%)    &    0 (0.00\%)     &   113 (15.7\%)    &    47 (5.58\%)    &    21 (8.94\%)    &    0 (0.00\%)     &    18 (6.41\%)    &    1 (0.61\%)     &    0 (0.00\%)     &    5 (8.06\%)     &    8 (14.0\%)     &    5 (8.93\%)     \\
    3 &    6 (0.49\%)     &    0 (0.00\%)     &    5 (0.69\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.61\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    4 &    0 (0.00\%)     &    0 (0.00\%)     &    1 (0.14\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
Child-Pugh stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    A &   810 (69.4\%)    &   1752 (88.0\%)   &   703 (85.1\%)    &   627 (74.5\%)    &   314 (79.7\%)    &   303 (95.0\%)    &   293 (98.0\%)    &   164 (99.4\%)    &    59 (77.6\%)    &    59 (93.7\%)    &    47 (82.5\%)    &    49 (87.5\%)    \\
    B &   307 (26.3\%)    &   239 (12.0\%)    &   117 (14.2\%)    &   215 (25.5\%)    &    78 (19.8\%)    &    13 (4.08\%)    &    6 (2.01\%)     &    1 (0.61\%)     &    17 (22.4\%)    &    4 (6.35\%)     &    10 (17.5\%)    &    7 (12.5\%)     \\
    C &    50 (4.28\%)    &    0 (0.00\%)     &    6 (0.73\%)     &    0 (0.00\%)     &    2 (0.51\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
mALBI\_stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    Grade 1 &   363 (33.2\%)    &   1498 (76.0\%)   &   331 (38.3\%)    &   289 (39.5\%)    &   145 (34.4\%)    &   210 (65.8\%)    &   225 (75.3\%)    &   126 (76.4\%)    &    26 (34.2\%)    &    36 (57.1\%)    &    32 (56.1\%)    &    26 (46.4\%)    \\
    Grade 2a &   274 (25.0\%)    &   292 (14.8\%)    &   204 (23.6\%)    &   202 (27.6\%)    &    96 (22.8\%)    &    72 (22.6\%)    &    50 (16.7\%)    &    27 (16.4\%)    &    15 (19.7\%)    &    16 (25.4\%)    &    6 (10.5\%)     &    10 (17.9\%)    \\
    Grade 2b &   392 (35.8\%)    &   172 (8.73\%)    &   238 (27.5\%)    &   220 (30.1\%)    &   171 (40.6\%)    &    35 (11.0\%)    &    23 (7.69\%)    &    11 (6.67\%)    &    29 (38.2\%)    &    10 (15.9\%)    &    17 (29.8\%)    &    19 (33.9\%)    \\
    Grade 3 &    66 (6.03\%)    &    8 (0.41\%)     &    92 (10.6\%)    &    21 (2.87\%)    &    9 (2.14\%)     &    2 (0.63\%)     &    1 (0.33\%)     &    1 (0.61\%)     &    6 (7.89\%)     &    1 (1.59\%)     &    2 (3.51\%)     &    1 (1.79\%)     \\
WBC (109/L), (median [IQR]) & 4.69 [3.47;6.26] & 5.11 [4.08;6.29] & 5.38 [4.20;7.40] & 5.50 [4.10;7.17] & 5.00 [3.80;6.30] & 5.60 [4.50;7.00] & 5.56 [4.50;7.04] & 5.18 [4.29;6.57] & 4.80 [3.88;6.15] & 6.26 [5.30;7.62] & 5.20 [3.40;6.40] & 4.55 [3.10;5.85] \\
NEUT (109/L), (median [IQR]) & 3.06 [2.12;4.50] & 2.86 [2.15;3.74] & 3.50 [2.40;5.68] & 3.40 [2.40;4.80] & 2.90 [2.16;4.10] & 3.57 [2.66;4.64] & 3.00 [2.40;4.15] & 3.24 [2.51;4.08] & 3.15 [2.40;4.60] & 3.89 [3.12;5.14] & 3.70 [2.50;4.70] & 3.25 [2.28;4.50] \\
LYMPH (109/L), (median [IQR]) & 1.01 [0.61;1.46] & 1.54 [1.19;1.96] & 1.17 [0.80;1.50] & 1.28 [0.88;1.74] & 1.30 [0.90;1.70] & 1.48 [1.07;1.85] & 1.68 [1.31;2.09] & 1.35 [1.02;1.71] & 0.90 [0.70;1.40] & 1.67 [1.30;2.03] & 1.10 [0.70;1.50] & 0.85 [0.60;1.20] \\
RBC (1012/L), (median [IQR]) & 4.03 [3.48;4.51] & 4.62 [4.23;4.98] & 4.09 [3.66;4.56] & 4.48 [3.92;5.00] & 4.06 [3.59;4.45] & 4.52 [4.12;4.88] & 4.70 [4.34;5.18] & 4.76 [4.40;5.11] & 4.40 [3.58;5.00] & 4.59 [4.25;4.86] & 4.40 [3.60;5.00] & 4.25 [3.18;4.82] \\
HGB (g/L), (median [IQR]) &  126 [110;139]   &  145 [133;155]   &  131 [116;142]   &  138 [123;152]   &  130 [118;143]   &  142 [128;154]   &  144 [128;154]   &  146 [133;156]   &  137 [120;152]   &  139 [126;145]   &  135 [120;150]   &  132 [115;147]   \\
PLT (109/L), (median [IQR]) &  135 [86.2;191]  &  153 [110;200]   &  154 [113;205]   &  158 [111;222]   &  124 [79.8;177]  &  156 [118;196]   &  184 [132;227]   &  160 [123;216]   &  159 [98.5;206]  &  220 [158;282]   &  152 [104;227]   &  148 [98.2;210]  \\
ALT (U/L), (median [IQR]) & 27.7 [17.6;47.4] & 25.0 [17.0;38.0] & 28.0 [18.0;47.0] & 35.0 [22.9;53.0] & 30.8 [21.0;45.7] & 30.0 [21.0;44.0] & 29.0 [22.0;41.0] & 30.1 [22.2;43.9] & 37.4 [24.0;51.4] & 31.0 [25.5;50.5] & 30.0 [15.8;43.1] & 32.2 [19.5;47.2] \\
AST (U/L), (median [IQR]) & 39.3 [25.0;78.3] & 26.0 [20.0;37.0] & 31.0 [22.0;46.0] & 42.0 [29.4;68.9] & 35.6 [25.0;54.8] & 34.0 [25.5;49.0] & 28.0 [22.0;40.0] & 31.9 [26.2;41.8] & 47.0 [31.5;70.7] & 42.0 [26.0;60.5] & 37.2 [27.4;67.0] & 44.9 [30.6;69.2] \\
TBIL ($\mu$mmol/L), (median [IQR]) & 15.3 [10.3;27.6] & 14.0 [10.3;18.7] & 15.6 [11.6;21.2] & 17.5 [12.7;24.1] & 18.1 [13.5;25.5] & 15.3 [11.7;20.4] & 13.3 [9.75;16.9] & 15.1 [12.1;19.6] & 18.9 [15.0;31.5] & 12.4 [8.15;18.8] & 16.2 [11.2;22.0] & 17.9 [10.9;28.1] \\
DBIL (umol/L), (median [IQR]) & 6.80 [4.60;14.2] & 5.50 [4.20;7.60] & 3.90 [2.70;6.10] & 6.70 [4.60;10.0] & 6.50 [4.40;10.1] & 3.10 [2.30;4.45] & 4.59 [3.50;6.06] & 2.83 [2.20;3.70] & 8.25 [5.65;17.5] & 4.10 [3.15;6.55] & 7.30 [4.40;12.4] & 6.90 [4.88;12.1] \\
ALB (g/L), (median [IQR]) & 37.1 [33.9;40.3] & 42.5 [39.7;45.4] & 38.3 [34.9;41.9] & 38.2 [35.3;42.0] & 37.7 [34.2;41.6] & 41.1 [38.7;43.5] & 42.2 [39.3;44.8] & 42.8 [39.8;45.8] & 37.8 [34.6;40.9] & 38.9 [36.0;41.9] & 40.6 [35.5;44.1] & 38.8 [35.0;43.2] \\
GGT (U/L), (median [IQR]) & 72.0 [37.0;162]  & 44.0 [27.0;79.0] & 58.5 [31.0;121]  & 96.0 [48.0;180]  & 59.0 [32.0;117]  & 53.0 [27.5;105]  & 41.0 [27.0;80.0] & 48.3 [29.0;95.5] &  107 [56.6;211]  &  106 [55.0;196]  & 97.5 [39.7;198]  & 95.7 [50.0;190]  \\
ALP (U/L), (median [IQR]) &  102 [76.0;152]  & 85.0 [69.0;108]  & 97.0 [76.0;132]  &  110 [84.5;160]  &  106 [78.0;146]  & 96.5 [78.0;128]  & 74.0 [61.0;94.0] & 93.1 [77.7;111]  &  135 [93.3;229]  &  110 [80.0;152]  &  114 [92.0;181]  &  118 [80.9;199]  \\
Cre ($\mu$mol/L), (median [IQR]) & 67.0 [57.0;78.0] & 69.0 [60.0;78.0] & 67.9 [59.3;78.7] & 67.0 [58.0;76.0] & 63.5 [55.1;73.7] & 71.4 [62.2;80.2] & 81.0 [68.0;93.0] & 75.8 [68.1;83.8] & 59.3 [51.8;71.6] & 73.0 [66.0;78.0] & 60.3 [51.4;69.0] & 65.4 [54.9;74.5] \\
BUN (mmol/L), (median [IQR]) & 5.00 [3.90;6.30] & 5.20 [4.30;6.20] & 5.21 [4.20;6.36] & 4.50 [3.60;5.70] & 4.75 [3.98;5.83] & 5.38 [4.38;6.43] & 4.90 [4.11;5.68] & 5.48 [4.50;6.33] & 4.90 [3.58;5.82] & 4.49 [3.37;5.46] & 5.10 [3.80;6.00] & 4.80 [4.05;5.90] \\
UA ($\mu$mol/L), (median [IQR]) &  308 [253;386]   &  306 [256;361]   &  301 [235;367]   &  311 [253;376]   &  271 [213;333]   &  323 [276;377]   &  315 [284;360]   &  346 [285;406]   &  298 [219;336]   &  320 [268;370]   &  299 [251;336]   &  287 [231;352]   \\
GLU (mmol/L), (median [IQR]) & 5.46 [4.87;7.26] & 5.25 [4.77;6.15] & 5.11 [4.58;6.18] & 5.38 [4.78;6.22] & 5.38 [4.84;6.20] & 5.58 [4.99;6.49] & 5.08 [4.89;5.72] & 5.28 [4.77;6.10] & 5.45 [4.90;6.50] & 5.80 [5.00;7.28] & 5.50 [5.00;6.40] & 5.60 [4.90;6.50] \\
PT (s), (median [IQR]) & 12.6 [11.9;14.2] & 11.9 [11.3;12.5] & 12.2 [11.4;13.0] & 13.1 [12.3;14.0] & 12.1 [11.3;12.9] & 13.2 [12.8;13.8] & 12.3 [11.7;13.0] & 11.7 [11.3;12.2] & 13.0 [12.0;13.9] & 11.9 [11.3;12.6] & 12.6 [11.8;13.9] & 12.9 [12.1;13.6] \\
INR, (median [IQR]) & 1.08 [1.02;1.23] & 1.03 [0.98;1.09] & 1.12 [1.04;1.19] & 1.04 [1.00;1.10] & 1.10 [1.04;1.19] & 1.02 [0.97;1.07] & 1.01 [0.96;1.06] & 1.04 [1.00;1.08] & 1.10 [1.00;1.20] & 1.05 [1.00;1.12] & 1.10 [1.00;1.20] & 1.10 [1.00;1.20] \\
APTT (s), (median [IQR]) & 28.8 [27.1;31.9] & 26.8 [24.9;29.3] & 31.3 [29.3;33.7] & 33.9 [28.5;37.7] & 34.1 [31.5;37.1] & 35.0 [33.0;37.8] & 32.3 [29.9;34.6] & 27.6 [26.2;29.0] & 28.6 [27.0;31.0] & 32.7 [30.7;34.6] & 27.7 [26.6;31.1] & 28.9 [27.1;30.9] \\
Fib (g/L), (median [IQR]) & 2.43 [1.82;3.18] & 2.55 [2.18;3.09] &  309 [248;393]   & 3.30 [2.68;4.11] & 2.66 [2.21;3.25] & 2.96 [2.42;3.57] & 2.81 [2.39;3.41] & 2.53 [2.20;2.97] & 3.55 [2.77;4.60] & 3.38 [2.81;4.07] & 3.50 [2.90;5.10] & 3.80 [2.90;4.95] \\
AFP, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    <=400 &   827 (78.5\%)    &   1608 (82.9\%)   &   578 (77.4\%)    &   259 (43.1\%)    &   341 (85.0\%)    &   238 (75.1\%)    &   235 (78.6\%)    &   115 (71.0\%)    &    33 (43.4\%)    &    37 (58.7\%)    &    26 (45.6\%)    &    18 (32.1\%)    \\
    >400 &   227 (21.5\%)    &   332 (17.1\%)    &   169 (22.6\%)    &   342 (56.9\%)    &    60 (15.0\%)    &    79 (24.9\%)    &    64 (21.4\%)    &    47 (29.0\%)    &    43 (56.6\%)    &    26 (41.3\%)    &    31 (54.4\%)    &    38 (67.9\%)    \\
PIVKA-II, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    <=1000 &   759 (73.6\%)    &   844 (85.7\%)    &   171 (65.8\%)    &   258 (45.9\%)    &      0 (.\%)      &   135 (79.4\%)    &    16 (72.7\%)    &   121 (76.6\%)    &    40 (52.6\%)    &    34 (54.0\%)    &    30 (52.6\%)    &    28 (50.0\%)    \\
    >1000 &   272 (26.4\%)    &   141 (14.3\%)    &    89 (34.2\%)    &   304 (54.1\%)    &      0 (.\%)      &    35 (20.6\%)    &    6 (27.3\%)     &    37 (23.4\%)    &    36 (47.4\%)    &    29 (46.0\%)    &    27 (47.4\%)    &    28 (50.0\%)    \\
Tumor numbers, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    1 &   675 (57.9\%)    &   1491 (75.3\%)   &   529 (75.5\%)    &   431 (52.5\%)    &   225 (66.8\%)    &   268 (84.3\%)    &   284 (95.0\%)    &   147 (89.1\%)    &    3 (3.95\%)     &    34 (54.8\%)    &    2 (3.51\%)     &    7 (12.5\%)     \\
    2 &   160 (13.7\%)    &   315 (15.9\%)    &   105 (15.0\%)    &    93 (11.3\%)    &    36 (10.7\%)    &    25 (7.86\%)    &    12 (4.01\%)    &    7 (4.24\%)     &    13 (17.1\%)    &    12 (19.4\%)    &    3 (5.26\%)     &    7 (12.5\%)     \\
    3 &    85 (7.29\%)    &    67 (3.38\%)    &    19 (2.71\%)    &    55 (6.70\%)    &    6 (1.78\%)     &    5 (1.57\%)     &    3 (1.00\%)     &    1 (0.61\%)     &    5 (6.58\%)     &    1 (1.61\%)     &    9 (15.8\%)     &    3 (5.36\%)     \\
    >=4 &   246 (21.1\%)    &   107 (5.40\%)    &    48 (6.85\%)    &   242 (29.5\%)    &    70 (20.8\%)    &    20 (6.29\%)    &    0 (0.00\%)     &    10 (6.06\%)    &    55 (72.4\%)    &    15 (24.2\%)    &    43 (75.4\%)    &    39 (69.6\%)    \\
Tumor maximum diameter, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    <=3 &   341 (29.8\%)    &   1023 (51.7\%)   &   161 (23.9\%)    &   150 (17.4\%)    &    90 (28.2\%)    &   120 (37.7\%)    &    97 (38.6\%)    &    48 (29.1\%)    &    3 (3.95\%)     &    12 (19.4\%)    &    3 (5.26\%)     &    6 (10.7\%)     \\
    >3, <=5 &   274 (23.9\%)    &   539 (27.3\%)    &   174 (25.8\%)    &   109 (12.6\%)    &    78 (24.5\%)    &    91 (28.6\%)    &    67 (26.7\%)    &    46 (27.9\%)    &    3 (3.95\%)     &    11 (17.7\%)    &    6 (10.5\%)     &    0 (0.00\%)     \\
    >5 &   531 (46.3\%)    &   415 (21.0\%)    &   340 (50.4\%)    &   605 (70.0\%)    &   151 (47.3\%)    &   107 (33.6\%)    &    87 (34.7\%)    &    71 (43.0\%)    &    70 (92.1\%)    &    39 (62.9\%)    &    48 (84.2\%)    &    50 (89.3\%)    \\
Vessel invasion, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   898 (75.7\%)    &   1901 (96.0\%)   &   453 (64.3\%)    &   471 (54.5\%)    &   182 (76.8\%)    &   301 (94.4\%)    &   291 (97.3\%)    &   125 (75.8\%)    &    24 (31.6\%)    &    50 (79.4\%)    &    18 (31.6\%)    &    16 (28.6\%)    \\
    Yes &   288 (24.3\%)    &    79 (3.99\%)    &   252 (35.7\%)    &   394 (45.5\%)    &    55 (23.2\%)    &    18 (5.64\%)    &    8 (2.68\%)     &    40 (24.2\%)    &    52 (68.4\%)    &    13 (20.6\%)    &    39 (68.4\%)    &    40 (71.4\%)    \\
Lymph Node Metastasis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   879 (87.8\%)    &   1738 (87.8\%)   &   603 (85.9\%)    &   800 (92.5\%)    &   378 (87.7\%)    &   314 (98.4\%)    &   295 (98.7\%)    &    165 (100\%)    &    70 (92.1\%)    &    55 (87.3\%)    &    48 (84.2\%)    &    49 (87.5\%)    \\
    Yes &   122 (12.2\%)    &   241 (12.2\%)    &    99 (14.1\%)    &    65 (7.51\%)    &    53 (12.3\%)    &    5 (1.57\%)     &    4 (1.34\%)     &    0 (0.00\%)     &    6 (7.89\%)     &    8 (12.7\%)     &    9 (15.8\%)     &    7 (12.5\%)     \\
Distant Metastasis, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   870 (86.1\%)    &   1926 (97.3\%)   &   636 (90.3\%)    &   757 (87.5\%)    &   376 (87.2\%)    &   317 (99.4\%)    &    299 (100\%)    &   162 (99.4\%)    &    62 (81.6\%)    &    52 (82.5\%)    &    35 (61.4\%)    &    45 (80.4\%)    \\
    Yes &   140 (13.9\%)    &    53 (2.68\%)    &    68 (9.66\%)    &   108 (12.5\%)    &    55 (12.8\%)    &    2 (0.63\%)     &    0 (0.00\%)     &    1 (0.61\%)     &    14 (18.4\%)    &    11 (17.5\%)    &    22 (38.6\%)    &    11 (19.6\%)    \\
BCLC stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    0 &    98 (9.91\%)    &   354 (17.9\%)    &    36 (5.68\%)    &    32 (3.80\%)    &    13 (5.51\%)    &    59 (18.5\%)    &    37 (14.7\%)    &    19 (11.7\%)    &    0 (0.00\%)     &    6 (9.68\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    A &   382 (38.6\%)    &   1068 (54.1\%)   &   249 (39.3\%)    &   264 (31.4\%)    &    92 (39.0\%)    &   199 (62.4\%)    &   195 (77.7\%)    &    95 (58.3\%)    &    0 (0.00\%)     &    20 (32.3\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
    B &   131 (13.2\%)    &   223 (11.3\%)    &    58 (9.15\%)    &   123 (14.6\%)    &    32 (13.6\%)    &    35 (11.0\%)    &    8 (3.19\%)     &    9 (5.52\%)     &    23 (30.3\%)    &    17 (27.4\%)    &    16 (28.1\%)    &    15 (26.8\%)    \\
    C &   328 (33.2\%)    &   329 (16.7\%)    &   285 (45.0\%)    &   423 (50.2\%)    &    97 (41.1\%)    &    23 (7.21\%)    &    11 (4.38\%)    &    40 (24.5\%)    &    53 (69.7\%)    &    19 (30.6\%)    &    41 (71.9\%)    &    41 (73.2\%)    \\
    D &    50 (5.06\%)    &    0 (0.00\%)     &    6 (0.95\%)     &    0 (0.00\%)     &    2 (0.85\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
CNLC stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    Ia &   300 (30.2\%)    &   1050 (53.2\%)   &   155 (24.3\%)    &   131 (15.6\%)    &    64 (27.1\%)    &   181 (56.7\%)    &   149 (59.4\%)    &    65 (39.9\%)    &    0 (0.00\%)     &    15 (24.2\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
    Ib &   179 (18.0\%)    &   372 (18.8\%)    &   128 (20.1\%)    &   165 (19.6\%)    &    41 (17.4\%)    &    77 (24.1\%)    &    83 (33.1\%)    &    49 (30.1\%)    &    0 (0.00\%)     &    11 (17.7\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
    IIa &    80 (8.06\%)    &   164 (8.31\%)    &    41 (6.44\%)    &    55 (6.53\%)    &    14 (5.93\%)    &    20 (6.27\%)    &    8 (3.19\%)     &    2 (1.23\%)     &    0 (0.00\%)     &    10 (16.1\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
    IIb &    51 (5.14\%)    &    59 (2.99\%)    &    16 (2.51\%)    &    68 (8.08\%)    &    18 (7.63\%)    &    15 (4.70\%)    &    0 (0.00\%)     &    7 (4.29\%)     &    23 (30.3\%)    &    7 (11.3\%)     &    16 (28.1\%)    &    15 (26.8\%)    \\
    IIIa &   152 (15.3\%)    &    50 (2.53\%)    &   178 (27.9\%)    &   282 (33.5\%)    &    34 (14.4\%)    &    16 (5.02\%)    &    7 (2.79\%)     &    39 (23.9\%)    &    36 (47.4\%)    &    6 (9.68\%)     &    16 (28.1\%)    &    28 (50.0\%)    \\
    IIIb &   175 (17.6\%)    &   279 (14.1\%)    &   107 (16.8\%)    &   141 (16.7\%)    &    63 (26.7\%)    &    7 (2.19\%)     &    4 (1.59\%)     &    1 (0.61\%)     &    17 (22.4\%)    &    12 (19.4\%)    &    25 (43.9\%)    &    13 (23.2\%)    \\
    IV &    56 (5.64\%)    &    0 (0.00\%)     &    12 (1.88\%)    &    0 (0.00\%)     &    2 (0.85\%)     &    3 (0.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    1 (1.61\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
TNM stage, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    IA &   105 (10.7\%)    &   354 (17.9\%)    &    36 (5.76\%)    &    32 (3.81\%)    &    13 (5.78\%)    &    60 (18.8\%)    &    37 (14.7\%)    &    19 (11.7\%)    &    0 (0.00\%)     &    6 (9.84\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    IB &   339 (34.6\%)    &   917 (46.5\%)    &   241 (38.6\%)    &   244 (29.0\%)    &    86 (38.2\%)    &   193 (60.5\%)    &   190 (75.7\%)    &    92 (56.4\%)    &    0 (0.00\%)     &    19 (31.1\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
    II &   138 (14.1\%)    &   285 (14.4\%)    &    38 (6.08\%)    &    59 (7.02\%)    &    20 (8.89\%)    &    25 (7.84\%)    &    11 (4.38\%)    &    12 (7.36\%)    &    2 (2.63\%)     &    7 (11.5\%)     &    1 (1.75\%)     &    4 (7.14\%)     \\
    IIIA &    64 (6.54\%)    &    89 (4.51\%)    &    30 (4.80\%)    &    84 (10.0\%)    &    16 (7.11\%)    &    18 (5.64\%)    &    2 (0.80\%)     &    0 (0.00\%)     &    21 (27.6\%)    &    11 (18.0\%)    &    15 (26.3\%)    &    11 (19.6\%)    \\
    IIIB &   166 (17.0\%)    &    50 (2.53\%)    &   178 (28.5\%)    &   282 (33.6\%)    &    34 (15.1\%)    &    16 (5.02\%)    &    7 (2.79\%)     &    39 (23.9\%)    &    36 (47.4\%)    &    6 (9.84\%)     &    16 (28.1\%)    &    28 (50.0\%)    \\
    IVA &    51 (5.21\%)    &   227 (11.5\%)    &    45 (7.20\%)    &    31 (3.69\%)    &    29 (12.9\%)    &    5 (1.57\%)     &    4 (1.59\%)     &    0 (0.00\%)     &    3 (3.95\%)     &    1 (1.64\%)     &    3 (5.26\%)     &    2 (3.57\%)     \\
    IVB &   116 (11.8\%)    &    52 (2.63\%)    &    57 (9.12\%)    &   108 (12.9\%)    &    27 (12.0\%)    &    2 (0.63\%)     &    0 (0.00\%)     &    1 (0.61\%)     &    14 (18.4\%)    &    11 (18.0\%)    &    22 (38.6\%)    &    11 (19.6\%)    \\
Surgery, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   635 (45.4\%)    &   866 (43.4\%)    &   309 (32.7\%)    &   323 (37.3\%)    &   323 (74.9\%)    &    30 (9.40\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    76 (100\%)     &    41 (65.1\%)    &    57 (100\%)     &    56 (100\%)     \\
    Yes &   763 (54.6\%)    &   1128 (56.6\%)   &   636 (67.3\%)    &   542 (62.7\%)    &   108 (25.1\%)    &   289 (90.6\%)    &    299 (100\%)    &    165 (100\%)    &    0 (0.00\%)     &    22 (34.9\%)    &    0 (0.00\%)     &    0 (0.00\%)     \\
RFA, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   1290 (92.3\%)   &   1209 (60.6\%)   &   902 (95.4\%)    &    865 (100\%)    &    431 (100\%)    &   303 (95.0\%)    &    299 (100\%)    &   116 (70.3\%)    &    76 (100\%)     &    58 (92.1\%)    &    57 (100\%)     &    56 (100\%)     \\
    Yes &   108 (7.73\%)    &   785 (39.4\%)    &    43 (4.55\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    16 (5.02\%)    &    0 (0.00\%)     &    49 (29.7\%)    &    0 (0.00\%)     &    5 (7.94\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
TACE, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   892 (63.8\%)    &   1914 (96.0\%)   &   863 (91.3\%)    &   679 (78.5\%)    &   108 (25.1\%)    &   302 (94.7\%)    &    299 (100\%)    &   159 (96.4\%)    &    30 (39.5\%)    &    34 (54.0\%)    &    22 (38.6\%)    &    22 (39.3\%)    \\
    Yes &   506 (36.2\%)    &    80 (4.01\%)    &    82 (8.68\%)    &   186 (21.5\%)    &   323 (74.9\%)    &    17 (5.33\%)    &    0 (0.00\%)     &    6 (3.64\%)     &    46 (60.5\%)    &    29 (46.0\%)    &    35 (61.4\%)    &    34 (60.7\%)    \\
HAIC, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   1181 (84.5\%)   &   1943 (97.4\%)   &   938 (99.3\%)    &   840 (97.1\%)    &    431 (100\%)    &   318 (99.7\%)    &    299 (100\%)    &   162 (98.2\%)    &    76 (100\%)     &    38 (60.3\%)    &    57 (100\%)     &    42 (75.0\%)    \\
    Yes &   217 (15.5\%)    &    51 (2.56\%)    &    7 (0.74\%)     &    25 (2.89\%)    &    0 (0.00\%)     &    1 (0.31\%)     &    0 (0.00\%)     &    3 (1.82\%)     &    0 (0.00\%)     &    25 (39.7\%)    &    0 (0.00\%)     &    14 (25.0\%)    \\
EBRT, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   1319 (94.3\%)   &   1994 (100\%)    &    945 (100\%)    &   542 (62.7\%)    &    431 (100\%)    &    319 (100\%)    &    299 (100\%)    &    165 (100\%)    &    0 (0.00\%)     &    63 (100\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
    Yes &    79 (5.65\%)    &    0 (0.00\%)     &    0 (0.00\%)     &   323 (37.3\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    76 (100\%)     &    0 (0.00\%)     &    57 (100\%)     &    56 (100\%)     \\
SIRT, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   976 (69.8\%)    &   1994 (100\%)    &    945 (100\%)    &    865 (100\%)    &    431 (100\%)    &    319 (100\%)    &    299 (100\%)    &    165 (100\%)    &    76 (100\%)     &    63 (100\%)     &    57 (100\%)     &    56 (100\%)     \\
    Yes &   422 (30.2\%)    &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     &    0 (0.00\%)     \\
TKI, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   972 (69.5\%)    &   1898 (95.2\%)   &   639 (67.6\%)    &   578 (66.8\%)    &   137 (31.8\%)    &   296 (92.8\%)    &   287 (96.0\%)    &    99 (60.0\%)    &    10 (13.2\%)    &    24 (38.1\%)    &    8 (14.0\%)     &    6 (10.7\%)     \\
    Yes &   426 (30.5\%)    &    96 (4.81\%)    &   306 (32.4\%)    &   287 (33.2\%)    &   294 (68.2\%)    &    23 (7.21\%)    &    12 (4.01\%)    &    66 (40.0\%)    &    66 (86.8\%)    &    39 (61.9\%)    &    49 (86.0\%)    &    50 (89.3\%)    \\
ICIs, n (\%) &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  &                  \\
    No &   1036 (74.1\%)   &   1887 (94.6\%)   &   663 (70.2\%)    &   591 (68.3\%)    &   143 (33.2\%)    &   260 (81.5\%)    &   287 (96.0\%)    &    89 (53.9\%)    &    14 (18.4\%)    &    28 (44.4\%)    &    12 (21.1\%)    &    12 (21.4\%)    \\
    Yes &   362 (25.9\%)    &   107 (5.37\%)    &   282 (29.8\%)    &   274 (31.7\%)    &   288 (66.8\%)    &    59 (18.5\%)    &    12 (4.01\%)    &    76 (46.1\%)    &    62 (81.6\%)    &    35 (55.6\%)    &    45 (78.9\%)    &    44 (78.6\%)    \\
 &  &  &  &  &  &  &  &  &  &  &  &  \\
Center A & Beijing Tsinghua Changgung Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center B & Tianjin Medical University Cancer Institute and Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center C & Zhongnan Hospital of Wuhan University &  &  &  &  &  &  &  &  &  &  &  \\
Center D & Mengchao Hepatobiliary Hospital of Fujian Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center E & Xingtai People's Hospital of Hebei Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center F & The Second Affiliated Hospital, Zhejiang University School of Medicine &  &  &  &  &  &  &  &  &  &  &  \\
Center G & Shenzhen People's Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center H & Southwest Hospital, Third Military Medical University (Army Medical University) &  &  &  &  &  &  &  &  &  &  &  \\
Center I & the Second Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center J & Guangxi Medical University First Affiliated Hospital &  &  &  &  &  &  &  &  &  &  &  \\
Center K & the Fourth Affiliated Hospital of Harbin Medical University &  &  &  &  &  &  &  &  &  &  &  \\
Center L & Peking Union Medical College Hospital &  &  &  &  &  &  &  &  &  &  &  \\
\end{longtable}
\end{center}
\end{landscape}



